Learning Efficient Disambiguation

This dissertation analyses the computational properties of current performance-models of natural language parsing, in particular Data Oriented Parsing (DOP), points out some of their major shortcomings and suggests suitable solutions. It provides proofs that various problems of probabilistic disambiguation are NP-Complete under instances of these performance-models, and it argues that none of these models accounts for attractive efficiency properties of human language processing in limited domains, e.g. that frequent inputs are usually processed faster than infrequent ones. The central hypothesis of this dissertation is that these shortcomings can be eliminated by specializing the performance-models to the limited domains. The dissertation addresses "grammar and model specialization" and presents a new framework, the Ambiguity-Reduction Specialization (ARS) framework, that formulates the necessary and sufficient conditions for successful specialization. The framework is instantiated into specialization algorithms and applied to specializing DOP. Novelties of these learning algorithms are 1) they limit the hypotheses-space to include only "safe" models, 2) are expressed as constrained optimization formulae that minimize the entropy of the training tree-bank given the specialized grammar, under the constraint that the size of the specialized model does not exceed a predefined maximum, and 3) they enable integrating the specialized model with the original one in a complementary manner. The dissertation provides experiments with initial implementations and compares the resulting Specialized DOP (SDOP) models to the original DOP models with encouraging results.

==> D-CH_DOPinML/Conclusions.tex <==
\subsection{Discussion of the analysis}
\label{ConcsDOPinML}
%The present chapter provides the common background, which the subsequent chapters
%depend on: Data Oriented Parsing (DOP), Bayesian-Learning, Explanation-Based Learning(EBL)
%and Entropy.
The section contributes a discussion of the DOP model as an 
algorithm for learning probabilistic grammars from tree-banks. This discussion  
\begin{itemize}
 \item relates DOP grammar-learning to EBL and Maximum-Likelihood (ML) learning,
 \item redefines the general framework of DOP in more solid terms,
 \item extracts, to some extent, the a priori knowledge, beyond the tree-bank,
       which DOP assumes in learning its grammar,
\end{itemize}
The present section, however, only initiates the research on DOP's learning element.
In this regard, future work may address, among others, some of the following
questions:
%
%\subsection{Open questions}
\begin{itemize}
\item
The discussion of the DOP framework as a learning algorithm raised an important
question for understanding why DOP works (when it does work). The question is:
{\em what assumptions does the DOP model make concerning the knowledge available to
the DOP grammar learner, besides the tree-bank, prior to learning~?}.
If we know exactly why DOP prefers some probabilistic grammar above others, we 
arrive at insights concerning the errors which a DOP grammar makes.
To my feeling, my attempt at answering this question, although illuminating, does not 
arrive at the desired deep answers. This question remains open. 
\item
 What can we say about the theoretical error rates, which a
 DOP grammar achieves~? It might be possible to state, for example, that DOP aims
 at optimizing some function of error on the training data.
%\item
% Under what circumstances is Bod's formalization of the DOP model a so called 
% ``consistent learner"~?
% A consistent learner learns the grammar which commits zero errors on the
% training tree-bank. Clearly, the DOP learning mechanism is not always a consistent 
% learner. The DOP STSG seems to select the choice, which minimizes some function
% of error on the training data, but it does not guarantee zero errors on the tree-bank.
% This is especially the case on ambiguous training sentences, where DOP resorts to
% probability for assigning an analysis to the sentence. This question is very much 
% related to the two preceding questions. 
%\item
%Is there, for every tree-bank, a grammar, smaller than the DOP STSG, which 
%is able to commit less errors than the DOP grammar on the tree-bank and on other
%sentences from the same domain~?
%\item
% For every tree-bank: is there an STSG, which has a string- and tree-languages 
% equal to those of the CFG underlying the tree-bank, and commits zero errors in
% assigning the most probable parse to the tree-bank sentences~?
\item
 One can easily simulate a Part of Speech-Tagging (PoSTag) n-gram model 
 using STSGs or SCFGs, even when the simulation is supposed to assign exactly 
 the same probabilities to the PoSTag sequences as the n-gram model.
 Surprisingly, it is not straightforward as it seems to find a DOP STSG\footnote{
 As mentioned earlier, the DOP STSG has all subtrees of the tree-bank as elementary-trees.
 And the probability of each of these elementary trees  is its relative frequency
 conditioned on its root label.
 }, which achieves this simulation. 
 To obtain a DOP STSG, one can attempt translating a corpus 
 of PosTagged sentences into a suitable tree-bank. However, it seems not possible to 
 obtain a tree-bank for which the DOP STSG assigns the same probabilities to all PoSTag
 sequences as the n-gram model. The combination of two features of n-gram models seems to
 prohibit this: 1)~n-gram models generalize recursively on sentence length in the training
 corpus, 2)~n-gram models assume that any syntax beyond PoSTags is of no influence at all 
 on the probabilities of PoSTag sequences and sentences. Due to these two features of n-grams,
 it seems that any attempt at obtaining a suitable tree-bank for training DOP to simulate
 an n-gram model will be unsuccessful; one of these two features is always sacrificed.
 Can a DOP STSG of some tree-bank simulate an n-gram model assigning the same probabilities
 to PoSTag sequences~?
\item How can a tree-bank annotation be generalized automatically in a manner 
   that does not jeopardize the probability distributions of the DOP STSG obtained from
   the generalized tree-bank~? (in fact, one's hope is even that there should be a  
   generalization that improves these distributions).
\end{itemize}


==> D-CH_DOPinML/D-figures/FigDOPINF.latex <==
\setlength{\unitlength}{0.00083300in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(9774,3699)(1339,-5023)
\thicklines
\put(1351,-5011){\framebox(2550,3525){}}
\put(6601,-2161){\line(-5,-2){1629.655}}
\put(4961,-2787){\line( 0,-1){993}}
\put(4961,-3780){\line( 3,-1){1656.300}}
\put(6616,-4336){\line( 0, 1){2175}}
\put(5110,-3367){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}Projection}}}
\put(5185,-3715){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}mechanism}}}
\put(7760,-2776){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}a}}}
\put(8736,-1921){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}S}}}
\put(8322,-2461){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}S}}}
\put(9460,-2416){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}b}}}
\put(8884,-2011){\line( 4,-1){521.882}}
\put(8884,-2011){\line(-5,-3){371.324}}
\put(8218,-2461){\line(-3,-2){222.231}}
\put(8662,-2836){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}et1}}}
\put(8292,-1711){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}0.25}}}
\put(10716,-3076){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}S}}}
\put(10154,-3556){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}a}}}
\put(10583,-3031){\line(-1,-1){283}}
\put(10361,-3886){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}et2}}}
\put(10139,-2761){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}0.50}}}
\put(9741,-4621){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}b}}}
\put(9283,-4006){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}S}}}
\put(8632,-4621){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}S}}}
\put(9268,-4171){\line(-2,-1){492.400}}
\put(9268,-4171){\line( 2,-1){421.200}}
\put(9105,-4936){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}et3}}}
\put(8736,-3811){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}0.25}}}
\put(2812,-4261){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}S}}}
\put(2251,-4726){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}a}}}
\put(2679,-4216){\line(-1,-1){275.500}}
\put(2531,-4006){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}t2}}}
\put(2916,-1951){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}S}}}
\put(3433,-2461){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}b}}}
\put(2295,-2506){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}S}}}
\put(1673,-2911){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}a}}}
\put(2857,-1996){\line(-3,-2){400.846}}
\put(2857,-1996){\line( 5,-2){518.103}}
\put(2162,-2476){\line(-4,-3){297.440}}
\put(2605,-1846){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}t1}}}
\put(3934,-3286){\vector( 1, 0){1108}}
\put(6666,-3286){\vector( 1, 0){1035}}
\put(7701,-5011){\framebox(3400,3675){}}
\put(5258,-3007){\makebox(0,0)[lb]{\smash{\SetFigFont{20}{24.0}{\rmdefault}{\bfdefault}{\updefault}DOP's}}}
\end{picture}


==> D-CH_Discussion/conclusions.tex <==
\chapter{Conclusions}



==> D-CH_GramSpec/AlgorithmsDef.tex <==
%%%%%%%%%%%%
%%%%%%%%%%%%
\newcommand{\COMSIZE}{}
\newcommand{\comment}[1]{{\COMSIZE\tt\bf ~/*~#1~~*/}}
\newcommand{\bcomment}[1]{{\COMSIZE\tt\bf ~/*~#1}}
\newcommand{\ecomment}[1]{{\COMSIZE\tt\bf ~#1~~*/}}
\newcommand{\EMPTY}{$\emptyset$}
\newcommand{\InBf}[1]{{\bf #1}}
\newcommand{\FUNC}{{\bf Function}~}
\newcommand{\BEGIN}{{\bf b}\={\bf egin}~}
\newcommand{\END}{{\bf end}~}
\newcommand{\UNION}{{\bf ${\bf \cup}$}~}
\newcommand{\REPEAT}{{\bf r}\={\bf epeat}~}
\newcommand{\UNTIL}{{\bf until}~}
\newcommand{\Set}{{\bf Set}~}
\newcommand{\TreeBank}{{\bf TreeBank}~}
\newcommand{\Integer}{{\bf Integer}~}
\newcommand{\bReturn}{{\bf return}~}
\newcommand{\bReturns}{{\bf returns}~}
\newcommand{\Boolean}{{\bf Boolean}~}
\newcommand{\For}{{\bf F}\={\bf or}~}
%%%%%%%%%%
\newcommand{\bREPEAT}{{\bf Repeat}}
\newcommand{\bUNTIL}{{\bf until}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THE ALGORITHM DEFINITIONS
\newcommand{\algScheme}{
\begin{figure*}[thb]
\hrule
{\sl
\begin{tabbing}
\comment{Let $N$ denote a unique address of a node of a tree $t$. Also let ${\TB}_{i}$ denote the}\\
\comment{tree-bank obtained after $i$ iterations, where ${\TB}_{0}$ denotes the given tree-bank.}\\ 
\comment{{\bf Frontier\_Of($N$)} denotes the frontier (i.e. an SSF) of the partial-tree under $N$.}\\
\comment{{\bf Descendent(Nch,Np)} denotes the predicate: the node addressed $Nch$ is a ~~~~~}\\
\comment{descendent of the node addressed $Np$.~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~}
%\comment{{\bf Max\_GRF($N$,$t$,$Set$)} denotes the predicate :}\\
%\comment{({\em ssf} := Frontier\_Of($N$)$ \in Set$) \AND~($\forall x \in Set$:~($x$ is competitor of {\em ssf} in $t$) $\rightarrow$ (GRF({\em ssf}) $\geq$ GRF($x$)) )}
\end{tabbing}
%
\begin{description}
\item [1.] $i := 0;$
\item [\bREPEAT]
\item [2.] 
\begin{tabbing}
$\forall$ \= $t\in {\TB}_{i}$, ~~$\forall$ node address $N$ in $t$:  N is {\it marked}\/ {\bf iff} \\
          \> Frontier\_Of(N) is SSF with 
                      sufficiently complete ambiguity set in ${\TB}_{i}$~ ~\AND \\
          \> ~~~$\forall$\=$Nx\neq N$ in $t$: ( Descendent(Nx,N) \OR Descendent(N,Nx) )~\lra~ (\MEAS(N) $>$ \MEAS(Nx)); 
\end{tabbing}
\item [{\bf 3.}] $i := i+1$;
\item [{\bf 4.}] ${\TB}_{i}$ := (${\TB}_{i-1}$ after reducing all partial-trees under marked nodes); 
\item [\bUNTIL] ((${\TB}_{i} == \emptyset$)  \OR~ (${\TB}_{i} == {\TB}_{i-1}$));
\end{description}
}
\hrule
\caption{The Learning Algorithm}
\label{LearnAlg}
\end{figure*}
}
%%%%%%%%%%%%


==> D-CH_GramSpec/D-ATIS-ExpRes/FigDepthToSize2.tex <==
\begin{figure}[htb]
\epsfxsize=13cm
\epsfbox{./D-CH_GramSpec/D-ATIS-ExpRes/depthgraphSize2.eps}
\caption{Number of subtrees to depth upper-bound (2nd experiment)}
\label{FigDepthUBSizeTwo}
\end{figure}


==> D-CH_GramSpec/D-ExpResults/FigATISExample.tex <==
\begin{figure}[hbt]
\center{
\begin{tabular}{c}
\epsfxsize=17cm
\epsfbox{./D-CH_GramSpec/D-ExpResults/trees1.ps}
\\
\epsfxsize=15cm
\epsfbox{./D-CH_GramSpec/D-ExpResults/trees2.ps}
\end{tabular}
}
\caption{ATIS examples of the transformations}
\label{FigDepthCPU}
\end{figure}


==> D-CH_GramSpec/D-ExpResults/d4D2meansTable.tex <==
{
\begin{table}[hbt]
%\hrule
%\begin{small}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
Measures & DOP$^{4}$  &  ISDOP$_{2}^{4}$  &  SDOP$^{2}$ \\
\hline
{\sl Recognized} &  95.25 (0.99) & 94.85 (1.42) & 91.45 (0.99) \\
{\sl TLC} & 89.60 (1.568) & 89.60 (1.568) & 89.60 (1.568) \\
Exact match &  89.35 (0.56) & 89.45 (1.55) & 91.30 (1.39) \\
Syn. ex. match &  94.90 (0.79) & 94.80 (0.79) & 96.30 (0.61) \\
Sem. ex. match &  89.90 (0.30) & 90.00 (1.30) & 91.50 (1.39) \\
NCB recall &  92.15 (1.51) & 91.30 (2.25) & 86.75 (1.55) \\
NCB prec. &  99.40 (0.21) & 99.35 (0.10) & 99.70 (0.05) \\
0-Crossing &  97.10 (0.72) & 96.90 (0.41) & 98.05 (0.34) \\
Syn. LBR &  91.45 (1.51) & 90.60 (2.06) & 86.35 (1.43) \\
Syn. LBP &  98.65 (0.29) & 98.55 (0.22) & 99.25 (0.15) \\
Sem. LBR &  90.05 (1.57) & 89.10 (2.03) & 85.20 (1.31) \\
Sem. LBP &  97.15 (0.36) & 96.90 (0.26) & 97.95 (0.26) \\
\# of sens &  685.75 (8.42) & 685.75 (8.42) & 685.75 (8.42) \\
Sen. length &  4.50 (0.03) & 4.50 (0.03) & 4.50 (0.03) \\
CPU (sec.) &  2.55 (0.23)  & 0.74 (0.09)  & 0.70 (0.03)  \\
\hline
\end{tabular}
\end{center}
%\end{small}
\caption{Means and stds of 5 partitions: sentence length $> 1$}
%\hrule
\label{Figd4D2meansTable}
\end{table}
}



==> D-CH_GramSpec/D-ExpResults/depthSizes.tex <==
model  d/D   #subs  #nodes
==========================
DOP    4    62571  2794928/8
DOP    5    91722  4895624/8
SPEC   2    
SPEC   5    52654  3164368/8


==> D-CH_GramSpec/D-ExpResults/plot6 <==
#set terminal latex
set terminal postscript eps "Times-Roman" 30
set data style points
set output "graph6.eps"
set size 1.3,1.3;
set xtics 1.0,1.0
set ytics 0.2,0.2
set format x "%g"
set format y "%2.2f"
set xlabel "-1*log(prob) for sentence length 6"
set ylabel ""
set xrange [1.2:22.0]
set yrange [0.0:4.1]
plot "merged.6" using 1:2 title "DOP" with lines 1,\
"merged.6" using 1:3 title "SDOP" with lines 5
#"dopD1d1CPU" t*100 title "DOP$^{1}$" with lines 4, \
#"specD1d1CPU" t*100 title "SDOP$^{1}$"  with lines 5, \
#"combD1d1CPU" t*100 title "ISDOP$_{1}^{1}$" with  lines 6
#
#
#
#"/home/simaan/D-Work/D-Experiments/D-AnalysisScripts/dop.CPU.table" title "DOP" with points,\
#"/home/simaan/D-Work/D-Experiments/D-AnalysisScripts/spec.CPU.table" title "SDOP" with points,\
#"/home/simaan/D-Work/D-Experiments/D-AnalysisScripts/comb.CPU.table" title "ISDOP" with points,\
###########
#"ProbsRes.log" title "result" with points
#set terminal latex
#set output "GraphStest.tex"
#set size 13/10., 15/20.
#set format x "$%g$"
#set format y "$%g$"
#set xlabel ""
#set ylabel "" -3, 2.5
#set xrange [-1:101]
#set yrange [-28.0:10.0]
#plot "zscore.test.s.num" title "test" with impulses ,\
#"zscore.Rtest.s.num" title "result" with points
#plot "probtest.log" title "test" with points ,\
#"probsres.log.num" title "result" with impulses 5
#plot "probtest.log" title "test" with points ,\
#"probsres.l.n.notnull" title "result" with impulses 1
#set terminal latex
#set output "Graph.tex"
#set size 6/5., 12/20.
#set format x "$%g$"
#set format y "$%g$"
#set xlabel ""
#set ylabel "" -3, 2.5
#set xrange [0:220]
#set yrange [-4.00:4.00]
#plot  "zscores.frag.sorted" title "" with impulses
#set terminal latex
#set output "Graph.tex"
#set size 6/5., 12/20.
#set format x "$%g$"
#set format y "$%g$"
#set xlabel ""
#set ylabel "" -3, 2.5
#set xrange [0:15]
#set yrange [-4.00:4.00]
#plot  "zscores.sq.sorted" title "" with impulses


==> D-CH_GramSpec/D-figures/Fig2old.tex <==
\begin{figure}[ht]
\epsfxsize=7.5cm
%ik wil om twee uur vertrekken
\epsfbox{./SimaanTrees2.eps}
\caption{Another tree from OVIS}
\label{ucombone}
\end{figure}
%%



==> D-CH_GramSpec/GRFwContext.tex <==
\item  [Context-sensitive $GRF$:]
      In computing the function \MEAS$()$ under the Reduction Factor regime
      (section~\ref{SecSpecAlgs}), for any sequence of symbols $S$:
      \mbox{\MEAS$(S) > 0$} iff \mbox{$CP(S) > \delta$}.
      Often however, due to data-sparseness,  the context-free requirement that 
      \mbox{$CP(S) > \delta$} is too rigid. Therefore, the implementation of the 
       Reduction Factor learning algorithm (section~\ref{SecSpecAlgs})
      employs a back-off technique on local context in the computation of the value 
      of \MEAS$(S)$. Here the local context is limited to two grammar symbols to the left 
      and two to the right of the sequence~$S$. 
   
      Let the operator ``$\cdot$" denote the infix concatenation operator on sequences of symbols.
      To achieve the back-off on local context also let:
      \begin{itemize}
      \item $C_{TB}(S)$ denote the set of all pairs (contexts) $\tuple{LC,RC}$, where $LC$
            and $RC$ are each a sequence of two grammar symbols, with which sequence $S$ is 
            encountered in tree-bank~$TB$. 
      \item $GC^{i}(S)$ denote the set of pairs $\tuple{GLC,GRC}$, where $0\leq i\leq 4$ 
            and $\tuple{GLC,GRC}$ is obtained from a context $\tuple{LC,RC}\in C_{TB}(S)$ by 
            replacing exactly $i$ symbols in \mbox{$LC\cdot RC$} by the wild-card symbol,
            a special symbol $*$ that matches any symbol of the grammar.
            Note that $GC^{4}(S)$ is the singleton set $\{\tuple{**,**}\}$ and that $GC^{0}(S)$ is
            in fact $C_{TB}(S)$. 

            If \mbox{$G = \tuple{GLC,GRC}$} is obtained from \mbox{$I=\tuple{LC,RC}$} by replacing 
            symbols with wild-cards, $G$ is called {\em a generalization}\/ of $I$ and 
            $I$ is called {\em an instance}\/ of $G$. Two contexts are called {\em unrelated}\/ 
            iff they are neither generalizations nor instances of one another.
            A context $C1$ is called {\em more general}\/ than context $C2$ iff $C1$ 
            contains more wild-cards than $C2$.
      \item $Viable(LC,S,RC)$  denote the proposition that is true iff the frequency 
            of $\tuple{LC\cdot S\cdot RC}$ exceeds the threshold $\Phi$
            and \mbox{$CP(LC,S,RC) > \delta$}, where $CP(LC,S,RC)$ is the Constituency 
            Probability of the sequence of symbols \mbox{$LC\cdot S\cdot RC$}. 
      \item $MGUVC(S)$ denote the set of Most General Unrelated Viable Contexts for 
            a sequence of symbols $S$ defined as follows
            \[ \tuple{LC,RC}\in MGUVC(S)~~ {\bf iff:} \]
            \begin{enumerate} 
              \item there is some $0\leq i\leq 4$ such that $\tuple{LC,RC}\in GC^{i}(S)$, 
              \item $Viable(LC,S,RC)$ is true, 
              \item \mbox{$\forall \tuple{LC1,RC1}\in MGUVC(S)$}: if $LC\neq LC1$ or $RC\neq RC1$
                    then $\tuple{LC,RC}$ and $\tuple{LC1,RC1}$ are unrelated, and 
              \item for every~$i$ and every $\tuple{LC1,RC1}\in GC^{i}(S)$, if $Viable(LC1,S,RC1)$ 
                    is true then $\tuple{LC1,RC1}$ is an instance of or identical to 
               $\tuple{LC,RC}$.
            \end{enumerate}
      \item
            \MEASG$(LC,S,RC)$ denote the following generalization of the original \MEAS$(S)$,
            where $\tuple{LC,RC}\in GC^{i}(S)$ for some \mbox{$0\leq i\leq 4$}:
\begin{tabbing}
~~~~~~~\= \bIf~ ($Viable(LC,S,RC)$ == false)~ \bThen~ \MEASG$(LC,S,RC) = 0$;\\
       \> \bElse~ \MEASG$(LC,S,RC) = GRF(LC\cdot S\cdot RC)$;\\
\end{tabbing}
         Note that if $\tuple{LC,RC}\in GC^{i}(S)$ for $i > 0$, then the frequencies of 
         \mbox{$\tuple{LC\cdot S\cdot RC}$} are the sums of the corresponding frequencies
         of the instances of $\tuple{LC,RC}$ in the set $GC^{0}(S)$.
      \end{itemize}
      Now we redefine the function \MEAS as:
        \[  \MEASM(S) = \sum_{\tuple{LC,RC}\in MGUVC(S)} \MEASGM(LC,S,RC) \]

      This redefinition sums over the GRF values of all unrelated most general context
      of the sequence~$S$. Note that in the case \mbox{$MGUVC(S) = \{\tuple{**,**}\}$} the value
      of this context-sensitive function $\MEASM(S)$ is equal to that of the 
      original $\MEAS(S)$. And in case $\tuple{**,**}$ is not $Viable$ then the new definition of
      \MEAS(S) backs-off to the set $MGUVC(S)$ of unrelated most general contexts 
      of $S$ that are viable.
\end{description}


==> D-CH_GramSpec/Neumann.tex <==
The background-theory in~\cite{Neumann94} is HPSG and the domain is
Appointment-Scheduling~\cite{UszkoreitEtAl94}. The operationality criteria
are of two types and are both manually specified: 
1)~syntactic criteria in the spirit of~\cite{SamuelssonRayner91}, and
2)~feature-structure uninstantiation criteria in the spirit of~\cite{SrinivasJoshi}.

In~\cite{Neumann94}, the tree-bank is assumed to contain HPSG-trees: each tree is 
a combination of a syntactic CFG-backbone-tree (shortly bare-tree) and a feature structure 
(with the correspondences between the nodes in the bare-tree and the features
in the feature structure). The learning process is not complicated and can be
summarized (with some minor simplifications) as follows:
\begin{enumerate}
\item The CFG-backbone-trees (shortly bare-trees) of the training HPSG-trees 
      are cut into partial-trees at some manually predefined syntactic categories,
\item The feature structures associated with every tree are then ``taken apart"
      such that with every bare partial-tree (resulting from the preceding step)
      the right feature structure remains associated,  
\item The features in the feature structures of a partial-tree 
      that correspond to substitution-sites at the frontier of the bare partial-tree
      are {\em uninstantiated}\/ by introducing suitable variables instead of their
      values.
\item The resulting partial-trees are stored in a discrimination-tree indexed by 
      the feature structures that correspond to the terminals on their frontiers.
      Note that partial-trees that have no terminals on their frontiers are not 
      indexed and are not used during the phase of applying the learned knowledge 
      to new input.
\end{itemize}
During the application phase, the words of the input sentence receive the corresponding
feature structure entries in the lexicon (after morphological analysis) and the resulting 
sequence is used as the index of the input sentence. For every part of the sentence the
discrimination-tree is traversed to retrieve the associated partial-trees. Subsequently,
the feature structures of the retrieved partial-trees are instantiated by (and unified with) 
the values found in the lexicon-entries of the words. The retrieved and instantiated 
partial-trees are stored in a Earley-type chart. However, rather than employing the fully
Earley-parser, Neumann employs a {\em deterministic}\/ Earley-type parser that prefers 
larger retrieved partial-trees to smaller ones; the algorithm neither backtracks nor 
computes the whole parse-space of the input sentence. He also describes a way to combine 
the specialized parser obtained by EBL with the original HPSG parser such that the 
retrieved partial-trees are completed by the HPSG-parser. However, this manner of combining 
the two parsers is based on a best-first search heuristic, 
i.e.\ it is not based on a quality of the specialization algorithm that enables complementary 
roles for the two parsers.


==> D-CH_GramSpec/Outline.tex <==
%-------------------------------------------------------
-Introduction:
 1. problem:  
    - About BCGs and the need for grammar specialization for domains.
    - Probabilistic pruning is a valid possibility for solving
      the problem. However, pruning is a technical solution which
      takes place only after generation of the to-be pruned partial-trees.
      An interesting question is how can domain bias really specialize 
      a BCG off-line. Of course this can still be combined with 
      probabilistic pruning; but while specialization affects the grammar
      (i.e. parser), pruning can be applied only during probabilistic
      evaluation i.e. disambiguation.
      Expected gains are: 1) speed, 2) improved probabilistic models based
                                       on the specialized grammar.
    - Conceptual two level systems: cheap parsing and expensive probabilistic disambiguation.

 2. history: history of grammar specialization using EBL;
   - what is EBL ? the utility problem and the need for measuring
     utility of learned knowledge or good indexing schemes of the
     learned knowledge.
   - mention Samuelsson's suggestion of combining EBL with inductive learning.
   - mention that there is some success with using EBL
%----------------- 
-Existing work on gram-spec. using EBL:
    Two kinds of EBL concepts: 
        1. Sentential, theory-based: 
              how all sentences should look like according to TAG.
              Theory dependent assumption.
        2. Phrasal, manually or automatically specified operationality criteria:
              In specific domains some of the phrasal-types can be considered 
              internal to others and in fact can be assumed not to generate at all
              or only in limited case.
    Two kinds of Learning:
        1. From one example, without any inductive bias, i.e. pure
           EBL's analytical learning (Srinivas, Rayner and early Samuelsson).
        2. EBL combined with statistical arguments i.e. augmenting EBL with
           inductive statistical learning (Samuelsson, Sima'an).

    Describe shortly each of the existing methods and its assumptions:
      - Rayner and Samuelsson
      - Samuelsson
      - Srinivas and Joshi
      - Sima'an
 
  Joint points of grammar-spec. (GS) of Rayner, Samuelsson and
	Srinivas are: 
 	1. use EBL (with or without augmentation with inductive learning)
 	2. speed-up is the goal and ambiguity reduction is a side effect 
 	3. trade of coverage for speed-up obtaining a completely new
    	   specialized grammar.
 	4. no elegant way to combine the learned grammar 
           with the original grammar
 	5. conceptually divide the parsing system into 
          a parser which generates the possible tree-space for
          the input, and a disambiguator which selects the preferred
          tree.

  Sima'an work disagrees with these works on: points 2, 3 and 4. In Simaan:
       1. A mixture of ambiguity reduction and speed-up is the goal
          using a heuristic measure.
       2. Learns a partial-grammar which can be combined with the
          original BCG in a elegant manner.
%-----------
Critique of existing work:
 1. (Srinivas & Joshi):
    EBL using knowledge of the grammar formalism (the theory
    underlying the parsing system): TAG people. 
    - limited application to TAG theory
    - results in limited coverage systems since it relies 
      heavily on an assumption on the structure of language which
      stems from a competence grammar. For example, when having a
      spoken language domain many phenomena shall remain uncovered.
    - two systems: one very fast with low coverage, one very slow
      with high coverage; 
    - Currently limited to learning on the sentential level only.
 2. (Rayner, Samuelsson):
    EBL by masking grammatical categories that are less productive,
    i.e. has minimal impact on coverage of the grammar: Rayner,
    Samuelsson and Carter. Here it results in a new specialized
    grammar that can generate and combine constituents only of some
    grammatical categories. 
    Features of this learning:
    - No guarantee of gain:
      Depends heavily on the assumption that there are in the domain 
      categories which can be masked without harming parse-space of 
      other categories badly. It is not guaranteed that the method
      will result in substantial improvement.
      The bright results of Samuelsson depend heavily on the prior 
      knowledge of the device (i.e. LR parser) that will use the grammar;
      good LR parser-table pre-compilation (i.e. good indexing of knowledge)
      is the main reason for the great speed-up achieved.
    - No guarantee of parse-space compatibility with the BCG:
      If a category is masked then other categories that depend on 
      it can produce some parses which might be necessary. 
      It is very hard to find a way to cover up on losses in the 
      parse-space due this category masking. This is because
      masked categories can not be compensated for or else it has
      no meaning to learn.
    - Limited to learning CFGs:
      No multiple derivations for the same parse allowed in the parser
      This implies that the learned grammar is simply again a
      Context-Free Grammar.
    - In Rayner's case: operationality criteria manually specified.
  3. Simaan:
    - An intuitively interesting heuristic which measures the utility 
      of learned knowledge but gives no guarantee of good results.
%----------------------------------------
-A new framework for grammar specialization:
 - Motivation
   - Definition of grammar specialization: Specialization, inherently, 
     implies an approach of removal of redundancy. Therefore we concentrate
     on ambiguity reduction in a direct manner.
   - We would like to learn from the tree-bank the grammar which represents
     the sentences of the tree-bank in the least ambiguous manner. 
     (- problem: do we end up overfitting to the tree-bank ? in that case
               we need some inductive bias which might be manually specified
               or be some principle such as the ``smallest" grammar or so)
   - Use a probabilistic framework for this: 
     - Bayesian Learning: describe it.
     - Entropy minimization: 
       - what is entropy and how can entropy measure the
         ambiguity of a grammar on a tree-bank.
       - what is the relationship between probability and entropy

 - some intuition on the algorithm: SSFs as constituents, sets of subtrees associated 
   with SSFs, what set of SSFs represents the tree-bank in the least ambiguous manner.
   ambiguity of an SSF as two decision step: bracket and then assign structure.
 - The learning algorithm with a generic utility function.
   The algorithm belongs to the ``sequential-covering algorithm" family: 
   ``learn a rule, remove the data it covers and then iterate this process".
 - example of a utility function: the Global Reduction Factor. 
 - Deriving the algorithm details when assuming entropy minimization.
 - Deriving the algorithm details when assuming Maximum Likelihood.


==> D-CH_Introduction/Introduction.tex <==
Humans interact in speech and in writing and they are able to understand the messages 
that they exchange. The main problem that keeps the researchers bussy in the field of Natural 
Language Processing (NLP) is how to model the linguistic capacity of humans.
Besides the ``elevated" scientific interest and curiosity, the research in NLP is
mostly driven and even financed by ``humble" market needs. People in the market dream of
the day when we can automate tasks in which language plays a central role, e.g. 
systems that you can command through speech, systems that are able to have a dialogue with 
humans in order to provide them with information and services such as time-table information
and ticket reservation, systems that translate the European Commission's lengthy reports 
simultaneously into fifteen or more languages. In fact some impoverished systems have already
found their way through to the market, e.g. dictation systems, speech-recognition systems 
that understand some words and even sentences. However, it is not at all an exaggeration
to say that the field of NLP is a baby that has just discovered that it can stand up (and then
immediately fall).

A major assumption that underlies the research in NLP is that all existing languages 
share a common internal structure.  This assumption is important because it implies 
that it is possible to capture the many and diverse languages in one single model. 
How this model should look like and what methods it should be based on is still a subject 
of debate in NLP research. However, most NLP researchers agree on the need for a 
divide-and-conquer modeling strategy: the model of understanding a spoken/written message 
is divided into a set of analysis modules, each dealing with a subtask of linguistic 
understanding. Examples of these analysis modules are speech-recognition, 
morphological analysis, part-of-speech tagging, syntactic analysis and semantic analysis. 
By dividing the complex task into smaller subtasks with suitable interfaces between them,
it becomes easier to develop solutions to each of the subtasks in isolation.

In this thesis we are only concerned with what are often seen as the last stages of
human understanding: syntactic and semantic analysis. Together these two are concerned with how 
to strip sentences, sequences of words, down to their internal structures that characterize
the meanings of these sentences. The syntax of a sentence is in fact a kind of skeleton
that supports the semantic flesh, i.e. the meaning, of the sentence. Usually syntactic 
analysis is considered as an inevitable ``fore-play" that prepares the sentence for 
semantic analysis.

%linguistics and competence
Linguistics has always been a major player in NLP research. In the last four decades of
linguistic research, the major concern has been to develop models that are able to
characterize what sentences are grammatical and how the meanings of these sentences 
are constructed from basic units; these basic units can be seen as the bits 
and pieces of the syntactic skeleton and the corresponding muscles of the semantic flesh. 
In this, linguistics has confined itself to studying how to describe a language as a set
of sentences, a set of analyses and the correspondence between instances of these two sets.
Usually, this triangle is described by a grammar that shows how sentences are constructed
from smaller phrases, e.g. verb-phrases and noun-phrases, that are in turn constructed from
yet smaller phrases or words. A grammar, thus, allows decomposing or {\em parsing}\/
a sentence into its basic units; the process of parsing a sentence using a grammar 
results in analyses. We say then that the grammar {\em assigns}\/ analyses to the sentence.
A linguist keeps herself bussy with finding out the type of grammars that seem most suited 
for describing languages and with studying hard linguistic phenomena. 

The focused interest of linguistics in developing grammatical descriptions has implied that
linguistics has not been interested in modeling the input-output behavior of language use 
by humans. Grammar engineering, an extension of theoretical linguistics, had the goal of
bridging the gap between theoretical linguistic research and research on how
to model input-output behavior. Grammar engineers use linguistic grammatical
descriptions for writing grammars that are aimed at capturing languages that consist
of non-idealized language use. All too often grammar engineers had to develop extensions
to linguistic grammatical descriptions in order to fill gaps in them. Despite of
these efforts, the developed grammars suffered from many problems among which two are
the most severe: overgeneration and undergeneration. Overgeneration,
also called the {\em ambiguity}\/ of a grammar, is the phenomenon that a grammar tends
to assign too many analyses to a sentence, most of which are not perceived by humans.
Undergeneration, on the other hand, is the phenomenon that a grammar does not assign
to a sentence the analyses that are perceived by humans (often the grammar does not assign
any analyses at all).

A grammar that undergenerates or overgenerates is not very useful in practice.
A system based on such a grammar tends to be brittle and inaccurate. Although some people
think that fiddling with the grammar rules might get things right, it is by no means
easy to get rid of overgeneration and undergeneration from a grammar for a serious portion 
of a natural language. In fact, there are no natural language grammars out there that cover
a domain without suffering from both problems. In this thesis we are interested in particular
in the problem of overgeneration, i.e.~ambiguity. 

% Ambiguity, what kinds of, examples and why is it a problem: how does it depend on
%        various sources (can you give examples ?)
% A different approach to performance models: learning from training material
% some examples from various fields of linguistics: HMMs for speech-recognition,
% HMMs and n-grams for PoSTagging, learned rules by Brill for PoSTagging, morphology by
% memory-based models etc.
% The probabilistic approach: what is the idea behind it ? 
% DOP: shortly 

%Problem statement of this thesis:


==> D-CH_Introduction/intro.tex <==
\chapter{Introduction}
\label{CHIntro}
%
\begin{verse}
 {\bf General short intro: problem, solutions, to whom the intro is written,
   the structure of the intro. }
\end{verse}
%
\section{Ambiguity and performance models}
Humans interact in speech and in writing and they are capable of understanding the messages 
that they exchange. The main problem that keeps the researchers bussy in the field of Natural 
Language Processing (NLP) is how to model the linguistic capacity of humans.
Besides the ``elevated" scientific interest and curiosity, the research in NLP is
also driven and often even financed by ``humble" market needs. People in the market dream of
the day when we can automate tasks in which language plays a central role, e.g. 
systems that you can command through speech, systems that are able to have a dialogue with 
humans in order to provide them with information and services (e.g.~time-table information
and ticket reservation), systems that translate the European Commission's lengthy reports 
simultaneously into fifteen or more languages. In fact some impoverished systems have already
found their way through to the market, e.g. dictation systems, speech-recognition systems 
that understand some words and even sentences. However, it is not at all an exaggeration
to say that the field of NLP is a baby that has just discovered that it can stand up (and then
immediately fall).

A major assumption that underlies the research in NLP is that all existing languages 
share a common internal structure.  This assumption is essential for NLP because it implies 
that it is possible to capture the many and diverse languages in one single model: the model
of human languages. 
How this model should look like and what methods it should be based on is still a subject 
of debate in NLP research. However, most NLP researchers agree on the need for a 
divide-and-conquer modeling strategy: the model of understanding a spoken/written message 
is divided into a set of modules, each dealing with a subtask of linguistic 
understanding. Examples of these modules are speech-recognition (constructing words 
from speech signals), morphological analysis (exposing the structure of words), 
part-of-speech tagging (categorizing words), syntactic analysis (exposing the structure
of sentences) and semantic analysis (assigning meanings to sentences). 
By dividing the complex task into smaller subtasks (with suitable interfaces between 
the corresponding modules), it becomes easier to develop solutions to each of the 
subtasks in isolation.

In this thesis we are mostly interested in syntactic analysis also called {\em parsing}.
% which is usually considered the preprocessor of the last stage of natural 
% language processing, i.e. semantic analysis. 
Together with semantic analysis, syntactic analysis is concerned with how to strip sentences 
down to their internal structures that characterize and expose the meanings of these sentences.
Syntactic analysis is considered by many as ``inevitable fore-play" that exposes the 
internal structure of the sentence for the ``real thing": semantic analysis. If we use 
anatomy as our model, the syntax of a sentence is a kind of skeleton that supports the 
semantic flesh of the sentence.

%linguistics and competence
\subsection{Competence and performance models}
Linguistics has always been a major player in NLP research to syntax and semantics. In the last 
four decades of linguistic research, the major concern has been to develop models that are 
able to characterize {\em what sentences are grammatical and how the meanings of these sentences 
are constructed from basic units}; these basic units can be seen as the bits 
and pieces of the syntactic skeleton and the corresponding muscles of the semantic flesh. 
In this, linguistics has confined itself to studying how to describe a language as a set
of sentences, a set of analyses and the correspondence between instances of these two sets.
Usually, this triangle is described by a grammar that shows how sentences are constructed
from smaller phrases, e.g. verb-phrases and noun-phrases, that are in turn constructed from
yet smaller phrases or words. A grammar, thus, allows decomposing or {\em parsing}\/
a sentence into its basic units; the process of parsing a sentence using a grammar 
results in analyses (we also say that the grammar (or a {\em parser}\/ that is based 
on it) {\em assigns}\/ analyses to the sentence).
A linguist keeps herself bussy with developing types of grammars that seem most suited 
for describing languages. For this hard task, the linguists had to make an inevitable
assumption as to what kind of language use interests them: linguists assume
that the subject matter of their studies is ``idealized" language such as that 
found in books. The linguists refer to the grammars that they develop as {\em competence}\/ 
models of language~\cite{Chomsky65}, as opposed to {\em performance}\/ models of language,
i.e. models of ``non-idealized" linguistic behavior of humans. 

\subsection{Overgeneration and undergeneration}
The focus of linguistics on developing grammatical descriptions has implied that
linguistics had no time for modeling {\em the input-output behavior of language use 
by humans}. Grammar engineering, an extension to (theoretical) linguistics, had the goal of
bridging the gap between theoretical linguistic research and research on how
to model input-output behavior. Grammar engineers (also linguists) use linguistic grammatical
descriptions for writing grammars that are aimed at capturing languages that consist
of non-idealized language use. All too often it turned out that the grammar 
engineers had to fill the many gaps in existing linguistic grammatical descriptions 
in order to make them fit the common language use in the applications they worked on.
Despite of the immense efforts, the developed grammars suffered from many problems among 
which two are most severe: overgeneration and undergeneration. Overgeneration,
also known as {\em ambiguity}, is the phenomenon that a grammar tends
to assign too many analyses to a sentence, most of which are not perceived by humans.
Undergeneration, on the other hand, is the phenomenon that a grammar does not assign
to a sentence the analyses that are perceived by humans (often the grammar does not assign
any analyses at all).

%{Ambiguity}
\input{./AmbigExamples}
Consider the sentence ``John found Mary a nice woman". It has two different interpretations:
{\em John considered Mary a nice woman}\/ or  {\em John searched and found for Mary a nice
woman}. Most people perceive only one interpretation (often the first). Nevertheless, it is
essential that a grammar of English be able to analyze this sentence both ways. Only within
enough context and with access to knowledge resources beyond language (world-knowledge) 
that the choice of the right analysis might become clear. A grammar engineer is assigned
the task of adjusting the linguistic grammars to resolve this and similar ambiguities.

Usually linguistic grammars assign to the preceding example sentence many other analyses
beside these two. Most analyses are not perceived by humans and are a byproduct of
the complex grammar rules. Consider for example the two sentences 
``Max eats Hommous with a fork" and ``Max eats Hommous with a bread". 
The meanings of both sentences are clear to the reader. The correct
syntactic analyses of both sentences are found in figure~\ref{FigAmbExamples}. 
Linguistic grammars are supposed to assign to each of the two sentences its correct
analysis. However, these grammars tend to assign to each of these sentences many analyses,
hopefully including the correct analyses. If the wrong analysis is assigned to a
sentence, it might result in the wrong meaning. Consider what happens if Max eats
the fork and the hommous; this is exactly what happens if the analysis at 
the right-side of figure~\ref{FigAmbExamples} is assigned to the sentence at 
the left-side of that figure\footnote{
Note that assigning the analysis of ``Max eats Hommous with a fork"  to ``Max eats Hommous
with a bread" implies using a bread to eat the Hommous, which is common practice 
in the Middle East and can be considered harmless. In any case, assigning any of the analyses
of these two sentences to  ``Max eats Hommous with a man" is equal to accusing Max of either
canebalism or slavery.}.
% Other examples of sentences that are assigned many analyses by linguistic grammar 
%are ``John is tall and handsome or popular" 
%(is he then {\em (tall and handsome) or poupular}\/ or is he {\em tall and (handsome or
%poular)}).
As mentioned above, linguistic grammars tend to assign many other analyses to these 
sentences that are never perceived by a human. In many cases these linguistic grammars 
assign hundreds but thousands of analyses to one sentence (see~\cite{MartinChurchPatil} 
for an empirical study of the problem).

A grammar that undergenerates or overgenerates is not very useful in practice.
A system based on such a grammar tends to be brittle and inaccurate. Sentences that are
assigned no analyses by the grammar are not understood by the system, and sentences that
are assigned too many analyses confuse the system. Many people thought (and very few
still think) that fiddling with the grammar rules might get things right. However, it is by 
no means easy to get rid of overgeneration and undergeneration from a grammar for a serious 
portion of a natural language. It is very hard for a human to keep track of the complex
interactions between the many rules of a grammar.
Even for the considerably much simpler task of writing
grammars for computer programming languages, getting rid of overgeneration and undergeneration is 
a very tedious job (sometimes with doubtful results as those who use the compilers notice). 
Usually, hacking the grammar to get rid of ambiguity immidiately results in extreme 
undergeneration (and vice versa); removing one analysis from the set that the grammar 
assigns to some sentence might imply that other sentences will miss their correct analyses. 
In fact, there are no serious natural language grammars out there that do not suffer from 
ambiguity as well as undergeneration.
%In this thesis we are in particular interested in one of these two problems:
%the problem of ambiguity.
\subsection{The probabilistic-linguistic approach}
A decade and a half ago a different approach to the problem of ambiguity in linguistic 
grammars revived due to its success in speech-recognition: the probabilistic approach. 
The slogan of this approach is: {\em allow linguistic grammars to overgenerate but resolve 
the ambiguities through assigning probabilities to the different analyses of a sentence}.
Assigning the correct probabilities to the analyses of a sentence enables  selecting one
analysis: the analysis with the largest probability. In fact, according to the probabilistic 
approach it is possible to assign such probabilities that minimize the chance of commiting 
errors in selecting an analysis\footnote{
A probabilistic model can minimize the chance of commiting error as much as it is
true to the task. If for example the probabilistic grammar is very shallow, e.g. sentences are
assigned only their categories (sentential-categories) without any internal structure, it  
can minimize the error of assigning to a sequence of words a sentential-category. The lower
bound on the error depends on how important really the internal structures that linguists 
assign to sentences for the task at hand. A good example of this scenario are the n-gram
models of part-of-speech tagging that seem to have a lower-bound on error (roughly 3-5\%).
}. Typically, assigning probabilities to the analyses is achieved by 
attaching probabilities to the rules of the linguistic grammar resulting in probabilistic 
or stochastic linguistic grammars 
e.g.~\cite{Fujisaki84,ViterbiCFG,Jelinek,Resnik,Schabes92,SchabesWaters93}

In one view on the probabilistic approach, the probabilities assigned to a linguistic 
grammar are considered means for modelling phenomena that the grammar is not aimed at 
modelling, e.g. broad-context (discourse) dependencies, world-knowledge. The probabilities, 
thus, constitute very fine grained means (i.e. averages) of many variables that influence 
the choice of the correct analysis of a sentence. Although this view is correct, this view
might not do the probabilistic approach full justice. Many people believe that the probabilistic 
approach to language has psychological evidence. A relevant psychological observation here 
is that {\em humans tend to register frequencies and differences between frequencies}.
Probabilistic models that employ relative frequencies can be seen as implementing
this observation on basis of Probability Theory. In any case, since here we are less 
interested in psychological studies, we will refrain from discussing them and we
refer the interested reader to the refrences cited in~\cite{Scha90,RENSDES}. 

\subsection{The corpus-based approach}
Although the probabilistic approach offers linguistic grammars a way out of the 
ambiguity maze, it does not offer a solution to the problem of developing performance
models of language. Linguistic grammars model idealized language use. Extending
them with probabilities does not make them suitable for modelling input-output linguistic
behaviour of humans. Many constructions will be missing from the linguistic grammar and
have to be engineered by humans. Moreover, there is a related fundamental question to
whether probabilities should be attached to linguistic grammar rules in the first place.
Generally speaking, probabilities are more meaningful when they are attached to dependencies
and relations that are more significant for the task they are imployed for. 
If you ask a linguist, she will point out that relations between words, between 
phrases and, for some sentences, even between whole constituents are often most significant 
in determining the correct analyses of sentences. Therefore, attaching probabilities to
the rules of a linguistic grammar is equivalent to attaching them only to a small portion
of the linguistic relations that are significant to syntactic and semantic analysis.

% A different approach to performance models: learning from training material
% some examples from various fields of linguistics: HMMs for speech-recognition,
% HMMs and n-grams for PoSTagging, learned rules by Brill for PoSTagging, morphology by
% memory-based models etc.

A major shift in developing performance models took place less than a decade ago.
It can be characterized as a shift from a {\em top-down}\/ approach to a {\em bottom-up}\/
approach to modelling. Rather than putting the linguistically developed competence models
central in performance models, the bottom-up approach puts collections of real-world data,
{\em corpora}, at the center of its activity. With the corpus of data at the center, 
this approach, the {\em corpus-based}\/ approach, aims at {\em acquiring}\/ or {\em learning}\/ 
from the data a suitable performance model. Crucially, the data is collected in such a way 
that it is representative of some language use in some domain.
The data might be {\em annotated}\/ with linguistic information, or it might 
be ``raw". If the data is annotated, the annotation is usually based on linguistic knowledge.
This offers  a  kind of ``back-door" where linguistic knowldge enters a performance model.
Learning from annotated data is analogus to tutoring (supervising) a novice in some task 
by showing them examples and their solutions. If the data is ``raw", this is similar 
to learning from scratch without the help of a supervisor (i.e. unsupervised learning).

By acquiring performance models from corpora, the corpus-based approach offers the
hope that the acquired performance models will be more suited for processing new similar data.  
Another attractive feature, market-wise, of automatic learning of performance models 
is the independence from manual labour, which is not always available and not always 
as consistent.

Currently, there are different corpus-based methods in linguistics.
Some of these methods have been successful in acquiring useful performance models for
some linguistic (relatively simple) tasks, e.g. part-of-speech tagging of free text (PoSTagging).
Example successful\footnote{There are also linguists that acquire their grammars and models 
from corpora manually, e.g. the Constraint-Based Grammar (CBG) approach~\cite{ENGCG}.
Though manually, this can be considered a linguistically-oriented corpus-based approach 
to acquiring linguistic models.
See~\cite{Samuelsson97} on a discussion of the role of linguistics in statistical 
learning and a summary of the CBG approach and where it (sensibly) meets and where it differs 
from other existing corpus-based approaches.} corpus-based methods for PoSTagging are Hidden 
Markov Models (HMMs)~\cite{BahlMercer76,Church88}, Transformation-Based Error 
Driven Learning~\cite{BrillPoSTagging,BrillThesis}, Instance-Based 
Learning~\cite{TilburgPoSTagging} and Maximum-Entropy Modelling~\cite{Ratnaparkhi96}.
Of course, there are a few more linguistic tasks for which 
the corpus-based approach currently offers suitable solutions, e.g. morphological analysis,
phonological analysis, chunking or recognition of noun-phrases. However, in general, these 
tasks constitute the less complex subtasks of sentence processing. For the more complex tasks,
e.g. syntactic and semantic analysis, none of the contemporary corpus-based approaches can 
claim similar success yet.

Most contemporary corpus-based methods to syntactic analysis are 
probabilistic, e.g.~\cite{SchabesIO,Magerman94,RENSDES,Charniak96,Collins96,Collins97,
Ratnaparkhi97,Srinivas97,GoodmanDES}; they acquire both their grammars and the probabilities 
of the grammars from {\em tree-banks}, i.e. corpora that contain syntactically analysed 
sentences. Some of these approaches achieve parsing accuracy that constitutes an improvement
even on well-developed linguistic grammars and parsers~\cite{Magerman94}. 
Nevertheless, none of these young methods has demonstrated yet that it is the most suitable. 
In this situation, the field of Computational Linguistics has become a kind of 
arena where young methods compete to prove their vitality and strength. No tools are spared
in this competition and every tool is welcome. Computational Linguistics is currently truely
a multidescplinary field where tools from many fields, e.g. Linguistics, Logic, Probability 
Theory, Information Theory, Computer Science and Machine Learning, are imported, sharpened and
accustomed for linguistic processing.
%
\section{Ambiguity and Data Oriented Parsing}
Data Oriented Parsing (DOP)~\cite{Scha90} is a performance model of language that 
is based on the observation that {\em adults tend to process linguistic input on basis
of their memory of past linguistic experience}. The linguistic experience of an adult is 
represented by a tree-bank of analysed sentences. To process new input, DOP relies on some 
psychological observations that boil down to the statement that 
``frequecies of analyses that are perceived in the past influence the choice of the 
analysis of the current input" (see~\cite{Scha90,RENSDES}). Thus, DOP does not only
memorize the past analyses but also their frequencies. To analyze a new sentence
DOP exploits similarities between this sentence and all sentences that occurred in 
the past. The frequencies of analyses that occurred in the past quantify the notion 
of similarity in DOP and allow the resolution of ambiguities.

DOP processes a new sentence by first recalling all relevant subanalyses of analyses from
the tree-bank. The notion of a subanalysis is taken here in the broadest sense: any part
of an analysis that does not violate the atomicity of grammar rules that constitute
that analysis. Then these subanalyses are assembled, in the same fashion as grammar
rules, into analyses for the current sentence. The process of assembling the subanalyses is
governed by their {\em relative frequencies}\/ in the tree-bank. In this process,
the relative frequencies are treated as probabilities and Probability Theory is brought 
into action for computing probabilities of assembled subanalyses and analyses. The most
suitable analysis for the current sentence is selected from among the many 
assembled analyses as the one with the largest probability.

The fact that DOP employs a memory of past experience relates DOP to a Machine 
Learning tradition with many names (and subtle differences): Memory-Based Learning, 
Analogy-Based Reasoning, Instance-Based Learning, Similarity-Based 
Learning (see~\cite{StanfillWaltz,Aha}). In fact, it is more interesting to notice that
DOP extends the Memory-Based tradition in two important ways: the analysis of new input 
does not rely on a flat representation of the past-analyses but on a deep linguistic 
structure of the analyses\footnote{This assumes a grammar as background-theory that provides 
the concepts, i.e. grammar categories, that enable the construction of the analyses.
These analyses are explanations, rather than flat classes, by the grammar on why it 
considers those sentences to be in the language it accepts.}, and the analogy function
is a probability function (with the relative frequency as interpretation of probability).
%
\section{This thesis}
This section states the problems that this thesis addresses and sketches the
solutions that it provides. 
%
\subsection{Problem statement}
This thesis deals with efficiency problems of contemporary performance models 
in general and the DOP model in particular. It studies and provides solutions for three
different problems. The first problem has to do with acquiring and applying these 
performance models under actual limitations on the available data, space and time.
This problem is most urgent in the DOP model and its various 
instantiations~\cite{RENS92,RENS95,Charniak96,SekineGrishman95,BonnemaEtAl97,BodKaplanSchaI}.
The second problem is that none of these models accounts for the desired property
that {\em more frequent input is processed more efficiently}. This problem 
is faced by all existing probabilistic grammars. And the third problem is that  
current performance models are not equipped to account for the fact that domain 
specific language use is less ambiguous than the general case.
Next, each of these problems is elaborated.\\
%
\begin{description}
\item [Problem~1:]
   Since performance models are meant for real-world language use, their natural habitat 
   is the world of applications. In general, the application of any performance model 
   to real tasks is governed by various limitations on space, time and data. Methods that 
   are not able to provide efficient solutions that fit into the available space and time 
   are impractical and will not scale up to larger applications. And methods that require
   huge ammounts of data are economically crippeled. This thesis addresses two aspects 
   of this problem that are particular to the DOP model (but apply also to other similar
   models):
    \begin{itemize}
      \item The Data Oriented Parsing algorithms developed prior to this 
         work\footnote{The first versions of the present work were published 
         in~1994~\cite{MyNEMLAP94}.} (Monte-Carlo parsing~\cite{RensMonteCarlo}) are 
         non-deterministic and are exponential time.  Parsing and disambiguation in 
         real-world applications (at least currently) can not be based on these methods.
         Moreover, these methods will not scale up to new larger applications.
         A related issue here is that prior to this work\footnote{Actually prior to    
         the work published in~\cite{MyCOLING96}.} there existed no studies
         of the computational time- and space-complexities of actual problems of disambiguation
         under the DOP model and similar probabilistic models.
      \item Some of the current performance models, in particular the DOP model, employ 
        very large probabilistic grammars. Due to the extensive size of these probabilistic 
        grammars, the following two problems arise with aquiring and employing them in practice:
 \begin{itemize}
    \item From a certain point on, the size of a probabilistic grammar becomes 
          a major factor in determining its efficiency. For real DOP probabilistic 
          grammars this is indeed the main factor that determines their actual time- and 
          space-consumption.
    \item The larger the probabilistic grammar, the more probability parameters it has.
          The more parameters a model has, the more data are necessary for acquiring 
          good relative frequencies as estimates of these parameters. This is the 
          problem of {\em data-sparseness}. Essentially this boils down to the economical
          observation that constructing larger tree-banks is expensive.
 \end{itemize}
    \end{itemize}
\item [Problem 2:]
    Existing performance models are not equipped with any mechanism that implements
     the desired property that more frequent input should be processed more efficiently. It is
     interesting to note that this property is sometimes attributed to human language 
     processing. Models that can not account for this property have suboptimal efficiency.
\item [Problem 3:]
 Many of the contemporary applications that involve natural language are aimed at specific
      language use that is determined by the domain of application, e.g. travel-information and 
      ticket-reservation systems, computer-manuals translators. An important observation about
      limited domains is that humans tend to express themselves in the same way most of 
      the time~\cite{WinogradFlores,SamuelssonThesis}. The direct implication of this 
      observation is that in such domains humans tend to employ only part of their linguistic 
      capacity. This is exactly the main motivation behind the various efforts at acquiring 
      grammars that are {\em specialized}\/ for limited 
      domains~\cite{Rayner88,SamuelssonRayner91,Samuelsson94,Srinivas97,Neumann94}.
      These efforts were directed to specializing linguistic broad-coverage grammars rather than
      full performance models that use probabilistic grammars. Their main goal was to acquire
      a specialized grammar with a limited but sufficient coverage (i.e. sentence recognition 
      power). For current performance models this does not {\em directly}\/ address the main 
      issue that domain specific language use is usually much less ambiguous than the 
      general case. 

     Existing performance models that are based on tree-bank annotated using 
     broad-coverage grammars are not equipped to account for the fact that domain 
     specific language use can be less ambiguous than the general case. This means 
     that essential knowledge from the tree-bank is missed when acquiring these 
     performance models.\\
\end{description}

One of the hypotheses that this thesis defends is that these problems are strongly
related. Especially the second and third problem can be integrated into one problem:
{\em more frequent and less ambiguous input in domain specific language use should 
be modelled as unambiguously as possible by a specialized performance model}. 
The property that more frequent input is processed more efficiently immidiately 
follows from this. If more frequent input is as unambiguous as possible then it is 
processed faster and it requires less space.
The third and the first problems are also related: when a probabilistic grammar is 
broad-coverage, it includes many probabilistic relations that are highly improbable 
in the domain. By specializing the probabilistic grammar and removing ambiguities that
are not domain specific, many of these relations are also removed from the probabilistic
grammar. This results in smaller probabilistic grammars and less parameters to estimate
from data.
%
\subsection{Sketch of solutions}
This thesis defends the idea that the main solution to these problems lies in 
employing two {\em complementary and interdependent}\/ systems for
ambiguity resolution in natural language parsing: 
%
\begin{enumerate}
\item An {\em off-line partial-disambiguation} system based on {\em grammar specialization
      through ambiguity reduction}. This system is acquired through the automatic learning 
      of a less ambiguous grammar from a tree-bank representing a specific domain. The main 
      goal here is to cash in on the measurable biases in that domain. The most important
      bias that the learning algorithm exploits is that more frequent and less ambiguous
      input is represented more efficiently.
\item An {\em on-line full-disambiguation} system represented by the DOP model. 
\end{enumerate}
%
These two manners of disambiguation are {\em complementary}: on-line disambiguation is applied
only where it is {\em impossible to disambiguate off-line without causing undergeneration}.
And, crucially, they are {\em interdependent}\/ since a specialized less ambiguous grammar, 
acquired off-line, can serve for {\em specialized}\/ re-annotation of the tree-bank;
a DOP model which obtained from this {\em specialized}\/ tree-bank is called a
{\em specialized DOP (SDOP) model}. 

For off-line disambiguation this thesis presents a new framework for the specialization
of DOP models and broad-coverage grammars dubbed the Ambiguity Reduction Specialization
(ARS) framework. For on-line disambiguation using the DOP model, this thesis presents
efficient deterministic polynomial-time and space algorithms. Important for the DOP model
is that these algorithms have time- and space-complexities that are linear in grammar-size.
Moreover, this thesis also presents a study of the computational complexity of some
problems of disambiguation under the DOP model and some existing probabilistic grammars. 
%
\section{Chapter description}
%According to these works, {\em specializing}\/ a given {\em linguistic grammar}\/
%to a given domain of language use is equivalent to acquiring a grammar that recognizes 
%only utterances from that domain. The {\em specialized grammar}\/ is, in this sense,
%a partial-grammar.


==> D-CH_OptAlg4DOP/D-back/CH_OptAlg4DOP.tex <==
\chapter{Efficient algorithms for DOP}
\label{CHOptAlg4DOP}
\input{./D-CH_OptAlg4DOP/Introduction}
\input{./D-CH_OptAlg4DOP/OthersAlgs}
\input{./D-CH_OptAlg4DOP/OptimizedAlg}
%\input{./D-CH_OptAlg4DOP/Experiments}
\input{./D-CH_OptAlg4DOP/Conclusion}


==> D-CH_OptAlg4DOP/D-back/Conclusion.tex <==
\section{Conclusion}
\label{SecConcs}
In this chapter we presented various deterministic polynomial-time algorithms for parsing
and disambiguation under the DOP model. We also presented optimizations of these algorithms 
that make them particularly suitable to deal efficiently with the DOP STSGs, which are typically
extremely large; in particular, these algorithms have time-complexity linear in STSG size 
at almost no extra memory cost. We also discussed various useful heuristics for projecting 
smaller and more feasible DOP STSGs from large tree-banks. 

The majority of the algorithms in this chapter were originally presented 
in~\cite{MyNEMLAP94,MyRANLP95} and later in an improved version in~\cite{MyRANLPBook}. 
Prior to the presentation of these algorithms, preceding work on DOP was unaware 
of the possibility of {\em deterministic polynomial-time}\/ parsing and disambiguation 
under STSGs in general and under DOP in particular.

The present algorithms have been implemented in an environment for
training DOP STSGs and parsing and disambiguation of sentences and word-graphs 
(i.e. SFSMs), dubbed the Data Oriented Parsing and Disambiguation System (DOPDIS).
%The heart of DOPDIS is the present optimized algorithm for computing 
%the MPD of an input sentence, and for computing the MPiD of an input word-graph under 
%an STSG.
%
Since their implementation in DOPDIS, the present algorithms have enabled
intensive monitoring of the behavior of the DOP model, a model that
was considered unattainable by many. The speedup that these algorithms achieve 
(in comparison to preceding Monte-Carlo~\cite{RENSDES}) is in the order of magnitude 
of hundreds of times (due to the optimized deterministic polynomial nature of the 
algorithms rather than to any implementation detail). This has made DOPDIS a very attractive 
experimentation-tool for other work involving DOP 
e.g.~\cite{BonnemaScr,BonnemaEtAl96,DOPNWORep,BonnemaEtAl97}.
Currently, DOPDIS serves as the kernel of the Speech-Understanding Environment of 
the Probabilistic Natural Language Processing~\cite{DOPNWORep} in the OVIS system,
developed in the priority programme Language and Speech Technology of the Dutch 
Organization for Scientific Research (NWO).


==> D-CH_OptAlg4DOP/D-back/Experiments.tex <==
\section{Empirical observations}
\label{SecEmpiric}
The experiments are:
\begin{verbatim}
For tasks: sentence/word-graph parsing and disambiguation
For domains: OVIS, SRI's-ATIS, maybe WSJ
Questions:
      0. quality of parse-space (how often is right parse in the parse-space)
      1. quality of MPD-parse
      2. upper-bound on quality of MPP-parse
      3. quality of probabilistic order of derivation-space (n-MPDs)
         maybe draw a graph: accuracy vs. the number of selected MPD's (n)

   Quality: for each experiment:
            1. exact match 
            2. labeled brackets accuracy and recall
            3. non-labeled brackets
            4. postagging quality
            5. exact sentence-match (for word-graphs)
            6. recall/accuracy words (for word-graphs)
     Also table of means and std

  Other measures:
         1. size of CFG/STSG in DOP STSG
         2. cpu-time CFG/STSG
\end{verbatim}

\subsection{OVIS sentences}
\subsection{OVIS word-graphs}
\subsection{SRI's ATIS sentences}
\subsection{Quality of approximations of the DOP model}
Allow probabilities to remain the same as in the USTSG rather than the limited-depth
DOP model: i.e. even for the limited model use the frequencies normalized with respect
to the whole space rather than the smaller space (this results in probability mass loss). 
Is there any significant change in accuracy ? this is a study of the quality of 
approximating the DOP model using the heuristics as well as the fact that original DOP 
only normalizes in the existence of all subtrees.
%
\subsection{Estimating MPP using MPD-algorithm}
Through retraining the subtrees we obtain new probabilities. How does this model
compare to DOP-MPD ?


==> D-CH_OptAlg4DOP/D-back/Heuristics.tex <==
%
\subsection{Successful heuristics}
For various domains and applications (e.g. speech understanding) 










 The sizes of the tree-banks we are facing are getting larger. The training trees are
 getting larger and more complex. So we need some useful ways to constrain the DOP
 models in a way similar to n-grams that are often limited to 3-grams or 2-grams.
 This is done by setting constraints on the form of the subtrees obtained from the
 tree-bank when obtaining a DOP model. Currently, within DOPDIS, we incorporated 
 the following four heuristics:
  1. upper bound on subtree depth (due to Bod) d_
  2. upper bound on number of subs sites in a subtree (Simaan) n_
  3. upper bound on number of words (terminals) in a subtree (Simaan) l_
  4. upper bound on number of adjacent words in a subtree (Simaan) L_
 These heuristics are combined in an AND when obtaining the subtrees.

 Extensive experiments has shown this, especially the depth and the sub sites
 upper bounds to be extremely effective in limiting the number of subtrees
 (list papers and reports showing this effect).

 Interesting points:
 - Why is the upper bound on num of subs-sites the least harmful when computing the MPD ?
    Simply because there is a strong association between the prob of a derivation
    and the number of substitutions that take place in it. So one can assume that
    for a given domain tree-bank there is an upper bound which does not harm the
    space of derivations or probabilities.
 
   One old experiment on ATIS words (without parsing unknown words).
   Showing that results achieved on ATIS are the same even when constraining the
   number of subs-sites. Maybe I should add more experiments ? on OVIS ? on large
   ATIS ?

 - Questions: Compute probability normalization in a constrained DOP grammar w.r.t.
       whole UTSG or w.r.t. constrained STSG DOP. Experiments to check this ?
   Discuss this and maybe show experiments on OVIS and ATIS ?
%%
%
\section{Empirical evaluation}
0.  What is the coverage possible i.e. how often is the right parse found in the
    parse forest anyway ?
1.  Is the probability of the right parse larger or smaller 
    than that of the MPD-predicted parse.
2.  How good are the n-MPDs in predicting the right parse ? 
%
Experiment with this on ATIS, OVIS, ATIS-SRI and maybe even WSJ.
Repeat every experiment 3 to 5 times with independent training/test sets.
%
%
\section{Discussion, open questions and suggestions}
1. Why does MPD work well for Phrase Structure Annotations in the tree-banks which we
  used for our experiments ? Can we provide an explanation for this ?
  Denote the order the parses of a sentence according to their MPDs with the term
  "MPD order of parse-space". Similarly define the ``MPP order of parse-space".
   It seems that under certain circumstances, for many sentences the top of the
   two orders is the same. What circumstances are these and can we derive this fact
   from these circumstances. Note that on the training set sentences the MPD of
   USTSG is equal to the MPP with high probability. 
   Possible observations: MPD is more prone to size of training-set, MPD is more prone
   to errors in training set.

2. When is MPD desirable more than MPP ?
   MPD becomes a better goal than MPP only when the notion of a derivation carries
   with it important clues which a naked parse does not: such as in TAG. Then training
   is done on derivations and parsing has the goal of computing the MPD rather than the
   MPP. The MPD carries a meaning for TAG, while the MPP does not.
3. Suggestion: online constraining of number of substitutions for computing MPD can
   speed up parsing without harming MPD accuracy.


==> D-CH_OptAlg4DOP/D-back/Introduction.tex <==
%{\tt Here a short predescription of the chapter}
%
Since its birth in~\cite{Scha90}, Data Oriented Parsing was considered by many as an unattainable
goal; interesting but only as a theoretical account of probabilistic disambiguation.
For many it was unthinkable that parsing natural language could take place on basis
of such huge probabilistic grammars. Bod was the first to run experiments~\cite{RENS1,RENSDES}
on the small Penn-Tree-bank ATIS (total of 750 trees). Bod's experiments raised conflicting
feelings: the reported accuracy results were ``good enough" to warrant the 
effort of looking into the model, but the fact that parsing one sentence took on 
average 3.5~hours seemed to support the argument that DOP is not feasible. 
In the absence of more efficient alternatives, Bod conducted these experiments using a 
Monte-Carlo algorithm~\cite{RENSMonteCarlo}, an approximation based on iterative random sampling, 
on Sun~Sparc~2 machines\footnote{
On the machines that are currently available (e.g. SGI~Indigo2) the average 3.5~hours 
per sentence would be reduced to about 20~minutes per sentence.}.
In retrospect, Bod can be credited for one thing: ``daring to look the beast in the eyes
with so much patience". 

Nevertheless, daring as they were, Bod's limited and unstable experiments %~\cite{GoodmanDES}
exhibit only the theoretical possibility of the Data Oriented Parsing approach.
They exhibit neither its feasibility nor its usefulness for real-life applications. 
In the world of applications, the natural habitat for performance models such as DOP,
there are various other requirements besides correct modeling. 
Efficiency is one major requirement: given 
the current limitations on space and time, what is the scope of applicability 
(e.g. language-domains, input-size, kind of application) of a given method~?

For DOP to be viable in the applications-world, it is necessary to have the 
algorithmic means that facilitate more efficient disambiguation. These algorithmic means
can be expected to go through various stages of development before they can achieve their
full potential. In this process of development, both the algorithms and the model are expected
to evolve: while the algorithms become more efficient, often they also reshape their models 
through acquiring new insights into these models. 

This chapter thus considers the question of how to disambiguate under DOP in 
an efficient manner. It provides efficient algorithmic solutions to some problems 
of disambiguation under DOP; typical to all these solutions is that they are, unlike
Monte-Carlo parsing, {\em deterministic polynomial-time and space}.
The present algorithms are ``pure" solutions, in the sense 
that they do not incorporate any assumptions or approximations that do not originate from
the DOP model. To improve the behavior of these algorithms in practice, this chapter
also presents approximations and heuristics that proved very effective and useful in
empirical studies of the DOP model. Some of these heuristics and approximations moderately
reshape the DOP model.
%
% This chapter also exhibits an extensive empirical study of the DOP 
%model on various domains, where the following questions play a central role: 
%\marginpar{HERE!!!}
%{\em 1)~how good does the MPD-selected parse disambiguate~? and 2)~does the MPP-selected 
%parse-tree constitute a potential improvement on the MPD-selected
%parse-tree with respect to the same measures of accuracy~?}. 
%Finally, independently of the answer to the previous question,
%the chapter also briefly discusses alternative means for approximating the 
%computation of the MPP under the DOP model; these alternatives try to circumvent
%the need for brute-force computation as in Monte-Carlo parsing.
%\marginpar{{\bf OOOO}}
%
%what is the upper-bound on the accuracy of the MPP, what is the accuracy of the MPD,
%what is the a~priori upper bound on accuracy, and how good does DOP order the derivations-space}.
%
\section{Motivation}
An important facility of probabilistic disambiguation is that it enables the selection of 
a single analysis of the input. Parsing and disambiguation of an
input under the DOP model can take place by means of maximization of the probability of some 
entity (in short ``maximization-entity"), e.g. for input sentences DOP could be made to 
select the Most Probable Parse (MPP), Most Probable Derivation (MPD) etc.. 
A central question in research on DOP has become the question: what entity should one
maximize~?
%
\subsection{What should we maximize~?}
In his presentation of the DOP model, Bod~\cite{RENSDES} singles out the MPP as the 
best choice for disambiguation under the DOP model when parsing input sentences. 
According to Bod, the MPP is, at least theoretically, superior to the MPD. This statement
is supported by some empirical results on the small Penn-TreeBank ATIS domain
(750 trees in total)~\cite{RENSDES,BodScha96}. 

The choice of the MPP, rather than the MPD, as maximization-entity is unique among 
existing probabilistic parsing models. Apparently this is due to the major role that SCFGs always 
played in these models: in SCFGs, there is no such difference between the MPD and the MPP
(since every derivation generates exactly one unique parse-tree). Theoretically speaking,
the MPP is superior to the MPD in the sense that it reduces the probability of commiting
errors. However, as we prove in chapter~\ref{CHComplexity}, the problem of computing the
MPP under STSGs is an NP-Complete problem. And, as we argue below, the existing 
non-deterministic algorithms (particularly Monte-Carlo parsing~\cite{RENSDES})
do not constitute practical solutions to this problem.
The crucial question that rises here is: is it always necessary to maximize the
theoretically most accurate entity~? In other words, are there situations when parsing
sentences where maximizing another entity than the MPP, e.g. the MPD, is sufficient~?

To answer this question we note first that in any situation the desired maximization 
entity should commit as little errors as possible. Generally speaking, error-rates are measured 
with respect to {\em subsequent interpretation of an analysis}; eventually, the interpretation 
module is the one that determines how fine-grained an analysis should be. And in its turn,
the amount of information contained in an analysis determines the kind of measure of error-rate
(e.g. exact-match, labeled bracketing precision).
In its turn, the measure of error determines the maximization entity that might be sufficient 
for the situation at hand. Clearly, in parsing sentences, whatever interpretation module 
we employ after parsing, the MPP remains the one that minimizes the chance of errors.
But there might be another entity that achieves as good (or comparable) results when the 
measure of error is less stringent than exact-tree match.

As a concrete example, consider the task of (non-labeled) bracketing
sentences. In such a task, one aims at minimizing the errors in assigning a bracketing 
to the input sentence. To this end, it is sufficient to maximize an entity that 
minimizes the chance of committing a wrong bracket. Although the MPP achieves this
goal perfectly, a less complex maximization entity achieves it equally well. 
This argument is the main motivation behind this and other work on developing efficient
algorithms for DOP~\cite{Goodman96,GoodmanDES}. 
%
\subsection{Accurate + efficient $\approx$ viable}
Bod's Monte-Carlo algorithm computes only {\em approximations}\/ of the 
Most Probable Derivation (MPD) and the Most Probable Parse (MPP) of an input sentence.
For achieving good approximations, it is necessary to apply the sampling procedure iteratively;
a quality of Monte-Carlo is that the result approaches the MPP/MPD as the number of iterations 
becomes larger. Bod claims that Monte-Carlo approximation is  {\em non-deterministic
polynomial-time}~\cite{RENSDES}; the polynomial is cubic in sentence length and square 
in error-rate. However, Goodman~\cite{GoodmanDES} argues\footnote{
Although the argument in~\cite{GoodmanDES} does not constitute a full proof, it is sound and
convincing. Goodman also constructed an efficient implementation of the Monte~Carlo algorithm.
For the small ATIS tree-bank~\cite{HemphilEtAl90} with 770~trees, Goodman  shows that 
this implementation runs (although exponential-time) as fast as his polynomial-time DOP 
parser (see below). Although this is a remarkable achievement, it is clear that this does
not necessarily scale up to larger tree-banks and longer sentences.
} that the error-rate in the time-complexity of the Monte-Carlo algorithm
is actually not a constant but rather a function of sentence length; 
this implies that Monte-Carlo parsing has in fact exponential time-complexity. 
%(defined as the difference between the probability of 
%the MPP/MPD and the probability of the Monte-Carlo approximation of it). 
Chapter~\ref{CHComplexity} supplies a proof that
the problem of computing the MPP for an input sentence under DOP is indeed NP-Complete,
making the Monte-Carlo algorithm one of the few ``brute-force" possibilities available. 

The fact that the Monte-Carlo algorithm obtains good approximations only when the number
of iterations is relatively large, makes it especially a prototyping-tool rather than 
a practical alternative. Future developments in multi-processor 
parallel computing and high-speed computing might change this but {\em only to a limited 
extent}. Given the fact that there will always be larger applications and larger domains,
it will always remain necessary to develop alternative efficient algorithms that constitute 
good solutions. As far as we can see, the presence of constraints on space and time is an
invariant in the evolution of computer programs. 
%And the notion of a {\em tractable problem}\/ 
%shall always remain: it designates a problem {\em that has such an algorithmic solution that 
%is most likely to be attainable under the given constraints of time and space}. 
Thus, if we wish to apply DOP within the given time and space limitations
rather than wait for a miracle to happen, we are obliged to develop efficient algorithms
for {\em as accurate as possible}\/ disambiguation under DOP. Of course, we are also obliged 
to remain aware of the ultimate accuracy of the original DOP model and strive for improving
the efficiency of the algorithmic means for achieving it.
%
\subsection{Efficient algorithms}
The goal of the present chapter is to present efficient and accurate algorithms for
disambiguation under large STSGs. We present: 
%
\begin{itemize}
 \item algorithms for computing the MPD under STSGs of an input 1)~parse-tree, 2)~sentence, 
       3)~FSM and 4)~SFSM (i.e. word-graph - see chapter~\ref{CHDOPinML}).
 \item algorithms for computing the probability under STSGs of an input 1)~parse-tree,
       2)~sentence, 3)~FSM and 4)~SFSM.
\end{itemize}
%
These algorithms are based on the same general algorithmic scheme.
Common to the present algorithms and other algorithms developed earlier within the
Tree-Adjoining Grammar (TAG) framework (see section~\ref{SecOthersAlgs})
is that they are all based on extensions of parsing and recognition algorithms that 
originally stem from the CFG tradition. 
The present algorithms differ from the algorithms developed in the TAG framework
in that they are two-phase (rather than single phase) algorithms. They are most suitable
for large DOP STSGs: their superiority is enhanced as the ratio between the size of 
the DOP STSG and the size of the CFG underlying it becomes larger, a typical
situation in natural language DOP STSGs.

In short, the present algorithms have two phases. The first phase spans a good 
{\em approximation}\/ of the parse-space of the input; this approximation is spanned 
by parsing under a simplified CFG that is an approximation of the CFG underlying the 
DOP STSG. The second phase computes the maximization entity (and the probabilities) 
on the parse-space that was spanned in the first phase.
Crucially, the parse-space spanned in the first phase constitutes a substantial limitation of 
the space that the DOP STSG would have to explore when parsing from scratch. Moreover,
in a typical DOP STSG, the CFG employed in the first phase is very small relative to the
large DOP STSG. Therefore, the costs of the first phase in space and time are negligible
relative to the second phase, and the second phase is computed in linear time-complexity
in grammar-size with as little ``failing" derivations as possible\footnote{
A common problem in parsing algorithms are actions taken by the algorithm that 
eventually do not lead to parses of the whole input but only to parses of part of the input.
These are often seen as failing derivations that cost time. Serious effort has been put into
reducing the failing derivations in CFG parsing as the next section explains.
}. The sum of the time/space costs of the two phases constitutes a substantial improvement
on the alternative one-phase algorithms. \\

The present algorithms compute the exact values rather than approximations as Monte-Carlo does.
Moreover, except for the algorithm for computing the MPD for an input sentence, none of these 
algorithms have been developed before within the Monte-Carlo framework.
In fact, for some of the above listed entities, it is highly questionable whether the 
Monte-Carlo algorithm can be adjusted to provide good approximations in reasonable 
computation-times (e.g. computing the probability of a parse-tree, a sentence 
or a word-graph).

An essential quality of the present algorithms, is that they have time-complexity 
linear in STSG size and cubic in input length. Crucially, linearity in STSG 
size is achieved without sacrificing memory-use, a typical situation in all other alternative 
algorithms that could be used for parsing DOP, 
e.g.~\cite{CKY,Earley,SchabesJoshi88,SchabesWaters93}. In section~\ref{CKYViterbi} I explain
why in the case of DOP STSGs the Cocke-Kasami-Younger (CKY) algorithm~\cite{CKY,AHO} does not 
succeed in providing
a good compromise between time and space needs for achieving time-complexity 
linear in STSG size. The same argument carries over to the other 
alternative algorithms that are listed above.\\ 

This chapter is structured as follows. Section~\ref{SecOthersAlgs} lists references to
and discusses related work on parsing and disambiguation under tree-grammars.
Section~\ref{CKYViterbi} mainly provides the background
to the rest of this chapter: it discusses CKY parsing under CFGs and the Viterbi optimization 
for computing the MPD/MPP of input sentences under SCFGs. It also argues that
the CKY algorithm and the Viterbi for CFGs are not suitable for parsing the huge DOP STSGs.
Section~\ref{SecOptAlg} presents deterministic polynomial-time algorithms and 
optimizations thereof.
Section~\ref{SecHeuristics} presents useful heuristics for improving the time- and
space-consumption of DOP models.
%Section~\ref{SecEmpiric} exhibits experiments and empirical results of parsing and disambiguation
%under DOP. 
And finally section~\ref{SecConcs} summarizes the conclusions of this chapter.
%with a brief summary and some open questions.
%This chapter presents the Data Oriented Parsing and Disambiguation System 
%(DOPDIS)~\cite{MyNEMLAP94,MyRANLP95,MyNEMLAPBook,MyRANLPBook,CLASKRep96}. 
%The heart of DOPDIS is an optimized  deterministic 
%polynomial time parsing and disambiguation algorithm suited for computing the
%Most Probable Derivation (MPD) and the Total Probability (TP) of an input sentence 
%or word-graph under an STSG. This algorithm, introduced in~\cite{MyNEMLAP94} and
%optimized in~\cite{MyRANLP95}, is the earliest deterministic polynomial time algorithm
%developed and applied for the DOP model. Prior to this algorithm, the DOP model
%had to resort to other non-deterministic polynomial time parsing methods such as
%Monte-Carlo Parsing~\cite{RENSMonteCarlo}. For DOP STSGs, the optimized version of 
%the algorithm is of (practically) linear time complexity in grammar size.
%
%DOPDIS is the first (and up till the moment of this writing) and sole complete
%system for training (i.e. parser generation), parsing and disambiguation for
%the DOP model.


==> D-CH_OptAlg4DOP/D-back/OlineOptAlg4DOP.tex <==
\chapter{An optimized algorithm for DOP}
\label{CHOptAlg4DOP}
% mention on what papers this chapter is based
THIS CHAPTER DEALS WITH COMPUTING THE  MPD under STSGs in general using an
optimized deterministic polynomial-time algorithm.
Also computing the probability of a given parse and the probability of
a given sentence. 

Based on the papers~\cite{MyNEMLAP94,MyRANLP95,MyRANLPBook,MyNEMLAPBook,CLASKRep,DOPNWORep}.
This chapter presents the DOPDIS system. The heart of DOPDIS is the 
optimized algorithms for computing the Most Probable Derivation (MPD)
and the Total Probability (TP) of an input sentence (or word-graph).
A short overview of DOPDIS.
DOPDIS is the first system for DOP that computes the MPD/TP
in a deterministic polynomial algorithm, linear is grammar size and up to
100 times faster than Rens's experiments on the same ATIS. DOPDIS is being
used within OVIS. 

%The parser+disambiguator-generator module containing a DOP training-module 
%and transformations of DOP trees into suitable data structures (the RB-STSG
%as presented in the algorithm). The parser module is a CKY parser for
%CFGs. The disambiguation module is based on an STSG probability computation 
%mechanism conducted on the CFG-parse space (maybe we need to mention some
%
\section{An optimized algorithm}
Present it as in the paper.
Improve the complexity analysis.
Exhibit original experiments of speed-up.
%
\section{Extension to word-graphs}
Short description of how to do this.
Provide complexity analysis. And include the number of transitions as
a constant.
%
\section{Extension with word-graph probabilities}
Show how to do this in relation to the optimized algorithm (the exact
place in the algorithm).
%
\section{Heuristic optimizations}
1. the useful d\_n\_l\_L .
2. the useful unknown words construction.
%
\section{Experimental results}
Exhibit the results on ATIS for sentences, on OVIS for sentences.
Show that n_2 in general provides the same results much faster.
For ATIS-SRI sentences and PoSTag sequences. Try WSJ experiments.
%
\section{Discussion and open questions}
1. What about TAG, can we use the same way to achieve faster algorithms ? Discussion.\\
2. Integrating pruning strategies: discuss some possibilities.


==> D-CH_OptAlg4DOP/D-back/OlineStructAll <==
  what the chapter presents: 
  Deterministic polynomial-time DOP algorithms
  MPD of a sentence, WG
  probability of a sentence, WG
  probabality of a partial-tree/tree

\section{Introduction}
  Problem description: 
     We are dealing with parsing and disambiguation (not mere recognition)
     Monte-Carlo alg is highly time consuming
     huge probabilistic grammars, so we need algs that are tailored for DOP
  A  possible algorithm, developed independently (Schabes-1993), for TAGs is
     R^2 N3 (can be R^n^3) and does not cash on the special structure 
     of language: relatively 
     small CFG description of the language that can be used to delimit the parse
     space even before very expensive disambiguation.
  In simaan-1994, an alg is described which cashes on this and in simaan-95...
     an algorithm of RN^3 is presented. Linear time in DOP grammar size has proved
     to be an essential part for practice and for experimentation with DOP.
  The system resulting from these algorithms is embedded in the DOPDIS environment.
  Describe DOPDIS and where it is being used.
  CHapter structure.

\section{An optimized polynomial-time algorithm}
  1. Present the MPD algorithm for word-graphs (without probabilities)
     and show how a sentence can be seen as a word-graph.
     a. Without optimization
     b. With optimization
  2. Also computing the prob of a sentence/wg on basis of that algorithm
  3. computing probability of a tree on basis of that algorithm
  4. Allowing speech-recognizer output word-graphs with probabs on the transitions
     (no empty transitions, no cycles). Show how that is done on basis of the algorithm
     above.
 
  One old experiment for showing speed up of linear algorithm.
%
\section{Successful Heuristic optimizations for MPD}
 The sizes of the tree-banks we are facing are getting larger. The training trees are
 getting larger and more complex. So we need some useful ways to constrain the DOP
 models in a way similar to n-grams that are often limited to 3-grams or 2-grams.
 This is done by setting constraints on the form of the subtrees obtained from the
 tree-bank when obtaining a DOP model. Currently, within DOPDIS, we incorporated 
 the following four heuristics:
  1. upper bound on subtree depth (due to Bod) d_
  2. upper bound on number of subs sites in a subtree (Simaan) n_
  3. upper bound on number of words (terminals) in a subtree (Simaan) l_
  4. upper bound on number of adjacent words in a subtree (Simaan) L_
 These heuristics are combined in an AND when obtaining the subtrees.

 Extensive experiments has shown this, especially the depth and the sub sites
 upper bounds to be extremely effective in limiting the number of subtrees
 (list papers and reports showing this effect).

 Interesting points:
 - Why is the upper bound on num of subs-sites the least harmful when computing the MPD ?
    Simply because there is a strong association between the prob of a derivation
    and the number of substitutions that take place in it. So one can assume that
    for a given domain tree-bank there is an upper bound which does not harm the
    space of derivations or probabilities.
 
   One old experiment on ATIS words (without parsing unknown words).
   Showing that results achieved on ATIS are the same even when constraining the
   number of subs-sites. Maybe I should add more experiments ? on OVIS ? on large
   ATIS ?

 - Questions: Compute probability normalization in a constrained DOP grammar w.r.t.
       whole UTSG or w.r.t. contrained STSG DOP. Experiments to check this ?
   Discuss this and maybe show experiments on OVIS and ATIS ?
%%
%
\section{Empirical evaluation}
0.  What is the coverage possible i.e. how often is the right parse found in the
    parse forest anyway ?
1.  Is the probability of the right parse larger or smaller 
    than that of the MPD-predicted parse.
2.  How good are the n-MPDs in predicting the right parse ? 
%
Experiment with this on ATIS, OVIS, ATIS-SRI and maybe even WSJ.
Repeat every experiment 3 to 5 times with independent training/test sets.
%
%
\section{Discussion, open questions and suggestions}
1. Why does MPD work well for Phrase Structure Annotations in the tree-banks which we
  used for our experiments ? Can we provide an explanation for this ?
  Denote the order the parses of a sentence according to their MPDs with the term
  "MPD order of parse-space". Similarly define the ``MPP order of parse-space".
   It seems that under certain circumstances, for many sentences the top of the
   two orders is the same. What circumstances are these and can we derive this fact
   from these circumstances. Note that on the training set sentences the MPD of
   USTSG is equal to the MPP with high probability. 
   Possible observations: MPD is more prone to size of training-set, MPD is more prone
   to errors in training set.

2. When is MPD desirable more than MPP ?
   MPD becomes a better goal than MPP only when the notion of a derivation carries
   with it important clues which a naked parse does not: such as in TAG. Then training
   is done on derivations and parsing has the goal of computing the MPD rather than the
   MPP. The MPD carries a meaning for TAG, while the MPP does not.
3. Suggestion: online constraining of number of substitutions for computing MPD can
   speed up parsing without harming MPD accuracy.


==> D-CH_OptAlg4DOP/D-back/OlineStructOptAlg <==
\section{An optimized algorithm for MPD}

\subsection{Background: CFG parsing with CYK}
% The CYK algorithm for CNF CFGs. That the algorithm is 
% in principle |R|n^3.
% Although CKY is indeed a parsing algorithm of |G|n^3
% there are various problems that lead to the fact that
% it behaves more like |G|^2. This is the case especially
% for non-CNF grammars that are very large.
%  1. transformation to CNF can lead to expanding the grammar
%   into G^2 (G is size of original grammar) (Gragham, Michael,
%    Harrison and Ruzzo 1980). The CKY is then |G|^2 in the 
%   original grammar rather than |G|
%  2. For achieving complexity |G| in CYK for CFGs we have to
%   use sets that can test membership and give access to members 
%   in O(1). This leads to substantial enlargement of memory-use
%   in practice (although in terms of O() both the |G| and the
%   |G|^2 algorithms have the same SPACE-complexity).
%
% How to apply the Viterbi for SCFGs MPD computation.
%  Its complexity: time and space.
%
\subsection{CYK for DOP STSGs: problems}
%  In principle, the CYK algorithm for CFGs can be applied
%   to TSGs of DOP directly if every subtree of the TSG is
%   treated as a rule ``root(subtree)-->frontier(subtree)".
%  However, in practice, due to the huge sizes of DOP
%  grammars the limitations of the linear time complexity in
%  grammar size of the CYK (mentioned above) become fatal.
%   
%  1. CNF transformation introduces as many as |A| new
%      non-terminals, and as many grammar rules.
%      This implies that each CKY entry will have the size equal
%      to the worst-case size |A| (to achieve linearity).
%      Although this does not change the worst-case complexity
%      in practice of NLP grammars this drastically enlarges
%      memory-use to the extent that it is often impossible
%      to run the parser !!
%       
%    To see why this is:
%     Let |GX| be the size of the TSG measured as follows:
%    for subtree A---->X1....Xt  size is 1+t
%    |GX| = tx|TSG|
%    When we transform the TSG into CNF, we want to preserve
%    the fact that the subtrees are units. So we have to
%    introduce, in the worst case, for every subtree new internal
%    nodes that are unique. For the above subtree we will introduce
%    t new non-terminals and also rules (with unique non-terminals 
%    carrying the subtree code). 
%  2. Another problem is the huge number of failing derivations
%     which such a grammar has. This implies extra work which does
%     not lead to parses.  This is of course inevitable in CFG parsing
%     but it is important to minimize it. Methods that use lookahead
%     variables and rely on knowledge of the grammar at hand can
%     reduce this a bit but for such a large TSG, this remains a burdain.
%     It is important to reduce this.
%

\subsection{A two-phase alternative parser}
%We present an alternative for DOP grammars that provides
%practical advantages over direct CYK TSG parsing for DOP
% grammars. Explain the parser in abstract terms.
% The parser is a two-phase parser. Firstly it
% spans an approximation of the parse-forest using an approximation
% ECNF grammar of the CFG (has slightly larger language than the
% CFG). In the second phase the parser applies fast recognition
% of the TSG deirvations on this parse-forest retrieving the
% wanted parse-forest. 
% Steps:
%  1. transform TSG subtrees into ECNF approximation.
%  2. Parsing on base of ECNF-CFG approximation
%  3. Recognition of TSG parses and MPD computation on 
%     parse-forest of previous step.
%
\subsubssection{ECNF approximation}
% Assume we need'nt care about the language of the TSG in
% transforming to ECNF. We only have to take care that we
% have a ECNF-CFG that has a language- and tree-sets that
% are supersets of the TSG language- and tree-sets.
% This can be achieved simply as we did in the implementation
%  EXPLAIN THIS shortly.
%  This transformation to CNF needn't expand the DOP grammar to |G|^2
%   We use a simplified, CFG-language expanding transformation,
%   i.e. a CNF-CFG approximation !! This does not expand the number
%   of non-terminals with more than |NT| non-terminals. The size of
%   the CFG is expanded by the number of non-terminal nodes added
%   to the CFG. This is in the worst-case maybe also |G|^2 but in
%   practice, due to introducing so few new non-terminals, many
%   rules collapse together and the number of rules is extremely
%   small compared to a full ECNF transformation that preserves the
%   language.
% 
\subsubsection{CYK parser for ECNF CFG}
% Shortly describe that and explain that it does not result in
% problems with the complexity of CYK for this CFG.
%
\subsubsection{TSG-derivations recognition and MPD computation}
% Our algorithm from the paper!!!
\subsubsection{Achieving almost linearity}
% The optimization of the TSG MPD computation.
\subsubsection{Advantages}
%0. We still achieve almost |A| time complexity without too
%   much memory-use:
%     Our parser is: |G|n^3 + |A||G|n^{3} = |A|x2x|G|x n^3
%     and this O(|A||G|n^3). Whenever |G| is extremely small
%     compared to |A| and n is large this becomes closer 
%     to O(|A|n^3) !!!
%  So now we can run experiments with huge TSGs very fast !! 
%     A thing that was almost impossible with the direct CYK
%     parser due to memory use in the |A| case. 
%1. No need for extensive use of memory in order to achieve
%   almost |G| time complexity. The rules of the TSG are the
%   subtrees: these are many. In usual CNF transformation
%   the number of different non-terminals in them is 
%   proportional to |NT|x|TSG|, where |NT| is number
%   of non-terminals in underlying CFG and |TSG| is number of
%   subtrees in the TSG. This is because, in order to recognize
%   subtrees we have to be able to recognize that subtrees are
%   units of CNF-CFG rules; this can be achieved only by marking the
%   CFG_CNF rules internal to each subtree with the number of the
%   subtree. This way we face a huge expansion of the memory-use needs.
%   By ECNF approximation this is avoided during the first phase.
%   In the second phase, due to the fact that the first phase 
%   delimits the TSG-parse-space, the application of this knowledge is
%   less bad and does not lead to huge entries.
%2. By parsing with CFG first, we reduce the void derivations
%   in the DOP grammar. Expected to give speed-up and spare memory.
%3. Further, conceptual clarity of a two phases: parsing followed
%    by probabilistic disambiguation. Also clarity of possibilities
%    for combining more linguistically adequate parsers with STSG
%    disambiguators becomes clearer.
%
\subsubsection{Disadvantages}
%1. Two phase parsing is expected to be slightly slower for relatively 
%    small TSGs and CFGs. So the parser is specialized in DOP.


==> D-CH_OptAlg4DOP/D-back/OptimizedAlg.tex <==
\section{Background: CKY and Viterbi for SCFGs}
\label{CKYViterbi}
In this section I discuss the classical CKY
algorithm for (deterministic) polynomial-time parsing of CFGs.
%I exhibit strong evidence that, in practice, direct use of this 
%algorithm for parsing DOP STSGs is 
%because it does not successfully compromise the two conflicting
%requirements of huge memory-needs and linear time-complexity in grammar size.
I argue that direct use of this algorithm for parsing DOP STSGs 
is impractical because it does not successfully compromise the two 
conflicting requirements of extensive memory-needs and high computation costs.
The direct application of the CKY algorithm for DOP is therefore
only a theoretical possibility.
%
\subsection{CFG parsing with CKY}
For the definition and notation of CFGs the reader is 
referred to chapter~\ref{CHDOPinML}. Some extra definitions and assumptions are necessary
here:
\begin{description}
%\item [CFG:]
%  Denote a CFG with the four tuple~\CFG, where \VN~ is the set of
%  non-terminals, \VT~ is the set of terminals, $S$ is the start non-terminal
%  and \Rules~ is the set of production rules (or simply rules). And let $V$ denote
%  \VN$\cup$\VT.
%\item [SCFG:] Denote an SCFG with~\SCFG, where \CFG is a CFG and 
%      \mbox{$P:\RulesN$\lra$(0,1]$} is a probability function. 
%\item [Notation:] $A, B, C, N, S$ denote non-terminal symbols and $a, b, c, w$ denote
%         terminal symbols, $\alpha, \beta, \gamma$ denote strings of 
%         symbols that can be either terminals or non-terminals. Adding numerical
%         subscripts to a symbol results in another symbol of the same type.
%         $w_{i}^{j}$ denotes the string of terminals \mbox{$w_{i}\cdots w_{j}$}.
%\item [Partial-derivation:]
%        The symbol $\lmd$ denotes a left-most {\em derivation (lmd) step} (or simply derivation
%        step), i.e. a relation
%         on \mbox{\VN$\mul V^{*}$} where a non-terminal symbol at the left-hand side (lhs)
%         of a rule from $\RulesN$~ is rewritten by the right-hand side (rhs) of that rule.
%         A (left-most) derivation is a sequence of derivation steps that starts with 
%         $S$ and terminates 
%         when there are only terminal symbols left over. A {\em partial-derivation}\/ is
%         any sequence of derivation steps.  The symbols \lmdir/\lmpdir~ denote respectively 
%         zero/one or more derivation steps (i.e. the first is the transitive and reflexive 
%         closure of $\lmd$ and the second is the transitive closure of $\lmd$). 
%\item [Partial-tree:] A partial-tree is a tree representation of a 
%        partial-derivation such that: 1)~the internal nodes of the tree are labeled with 
%        non-terminals and the leaf nodes are labeled either with terminals or non-terminals,
%        2)~if $X$ is the label of the parent of the nodes labeled with $X_{1}\cdots X_{m}$ 
%        then there is a rule $\RuleM{X}{X_{1}\cdots X_{m}} \in \RulesN$,
%        and 3)~the partial-derivation can be retrieved from the partial-tree if the rules are 
%        read of the partial-tree by a traversal starting at the root, where first
%        the label is read of the current node then the traversal is applied depth-first
%        to the children in turn from left to right. The partial-tree is said to be generated
%        by the partial-derivation it represents. A partial-tree is often also called a
%        partial-parse tree or simply partial-parse. 
%        In particular, a {\em parse-tree}, or parse or tree, is the partial-tree generated by 
%        a derivation.
\item [CNF:] 
  To simplify the presentation of CKY we assume CFGs in Chomsky Normal Form (CNF);
  a CFG is said to be in CNF iff each of its rules
  is in one of two possible forms: the binary form $\RuleM{A}{B C}$ or 
  the terminal form $\RuleM{A}{a}$.
\item [Sizes:] $|X|$ denotes the cardinality of a given set $X$.
       $|\alpha|$~denotes the number of symbols in string $\alpha$.
       And $|G|$~denotes the size of a CFG $G$=\CFG, not necessarily in CNF,
       where by definition:
        $|G|$=\mbox{$\sum_{\RuleM{A}{\alpha}\in \RulesN}  |\alpha| + 1$}.
\item [Finitely ambiguous:]
   Throughout this work we assume that the CFGs we deal with are {\em finitely ambiguous}\/
   i.e. the CFG derives any finite string it can recognize only in a finite
   number of different left-most derivations\footnote{This is equivalent to saying that the
   CFG does not allow cycles, e.g. $A$\lmpdir$A$.}. 
\item [Items:] In parsing theory, an item is a CFG rule with a dot inserted 
            somewhere in its right-hand side,
             e.g. \ITEM{A}{\alpha}{\beta} where $\RuleM{A}{\alpha\beta}\in$ \Rules. 
            Items \ITEM{A}{\alpha}{} are called final. 
            Roughly speaking, in general, the dot in the item
            is a marker, which identifies the stage of a derivation beginning from the rule
            underlying the item:
            $\alpha$ is the part already recognized and $\beta$ is the part that still 
            has to be recognized. In the following characterization of the CKY algorithm
            we show exactly what the dot marks.
\end{description}
%
The CKY algorithm~\cite{CKY} is one of the earliest and simplest algorithms
for polynomial-time recognition of arbitrary Context-Free Languages (CFLs). CKY
employs a data-structure, called well-formedness table, with entries $[i,j]$ for
all $0\leq i < j\leq n$, where $n$ is the number of terminals in the input
sentence. An entry is a store of items that are introduced during the parsing process.
Let \mbox{$w_{1}\cdots w_{n}$} denote the input sentence, and let $w_{0}=\epsilon$.
The invariant of CKY is to maintain the following condition for every 
entry $[i,j]$ in the table at all times:
%
\begin{verse}
  \ITEM{A}{\alpha}{\beta}$\in [i,j]$ iff 
  \mbox{$\RuleM{A}{\alpha\beta}$ \lmdir $w_{i}^{j}\beta$}\/ holds in the CFG at hand.
\end{verse}
%
This condition implicitly explains the notation of an item; CKY recognizes the 
input sentence iff there is an item \ITEM{S}{\alpha}{} in entry $[0,n]$. 

A specification\footnote{
This specification is rather inefficient. It does not optimize the order 
of steps of the CKY parser. 
} of the CKY algorithm is given in figure~\ref{FigCKYAlg}.
For more information on the CKY and on how to implement it efficiently, the reader is 
referred to~\cite{AHO,GrahamEtAl80}.
%
\begin{figure}
\hrule
\begin{tabbing}
{\bf Init:} \=                                           \\
            \>$\forall$~ \= $0 < i \leq n$  	 \\
            \>           \> $\forall$ \= ~$\RuleM{A}{w_{i}} \in$ \Rules      \\
            \>           \>           \> ~~~add \ITEM{A}{w_{i}}{} to $[i-1,i]$ \\
            \>           \> $\forall$ \= ~$\ITEMN{B}{\beta}{} \in [i-1, i]$  \AND~ $\forall~ \RuleM{A}{B C} \in$ \Rules \\
            \>          \>            \> ~~~add \ITEM{A}{B}{C} to $[i-1, i]$  \\
{\bf Deduce:}\=                  					\\
             \>$\forall~ 0 \leq i < n$       			\\
             \>$\forall$~\= $i < j \leq n$			\\
             \>          \> ~~~$\forall$\= ~$i < k < j$  \AND~  $\forall$~ \ITEM{A}{B}{C}$\in [i, i+k]$ 		\\
             \>          \>             \> ~~~~~\bIf~ $\exists$ \ITEM{C}{\alpha}{} $\in [i+k, j]$\\
             \>          \>             \> ~~~~~\bThen~ add \ITEM{A}{BC} to $[i, j]$ \\
             \>          \> ~~~$\forall$ \= ~$\ITEMN{B}{\beta}{} \in [i, j]$  \AND~ $\forall~ \RuleM{A}{B C} \in$ \Rules \\
             \>          \>              \> ~~~~~add \ITEM{A}{B}{C} to $[i, j]$  \\
\end{tabbing}
\hrule
\caption{CKY algorithm for CFGs in CNF}
\label{FigCKYAlg}
\end{figure}
%
As figure~\ref{FigCKYAlg} shows, the CKY {\em recognition}\/ algorithm has time-complexity 
proportional to $|G|\mul n^{3}$. However, to achieve time-complexity linear in grammar 
size $|G|$ it is necessary to be able to decide on the membership condition 
               ``if \mbox{$\exists$ \ITEM{C}{\alpha}{}$ \in [i+k, j]$}"
in $O(1)$. This is easily achieveable using very efficient implementations of entries
as arrays. Note that such an array, however, has to be of size $|V_{N}|$~ in order to
allow this. Good hashing functions approximate this behaviour using smaller arrays or 
lists.
%
\begin{figure}
\begin{center}
\mbox{
\epsfxsize=130mm
\epsfbox{./D-CH_OptAlg4DOP/D-figures/AddedBySet.eps}
}
\end{center}
\caption{Illustration of a possible implementation of a parse-forest} 
\label{FigAddedBySet}
\end{figure}
%

The recognition algorithm is in itself not very useful since it does not offer an 
efficient way for retrieving parse-trees for the input sentence. For this reason, 
the algorithm is usually extended at the {\bf Deduce} phase as follows: when adding item 
$I$ to entry \entry{i}{j}, a set of ``pointers", referred to as
$AddedBySet_{I, i, j}$, is attached to item $I$ (see illustration in figure~\ref{FigAddedBySet}). 
Each pointer in $AddedBySet_{I, i, j}$
points to an item in an entry \entry{k}{j} that resulted in adding $I$ to \entry{i}{j}
during the {\bf Deduce} phase of the algorithm. Note that a final binary item \ITEM{A}{BC}{}
is added to \entry{i}{j} by pairs of items \ITEM{A}{B}{C} $\in$ \entry{i}{i+k} and 
\ITEM{C}{\gamma}{} $\in$ \entry{i+k}{j}; therefore, $AddedBySets$ of final binary items 
are always pairs of pointers. For simplicity we refer to 
$AddedBySet_{I, i,j }$ as the $AddedBy$ set of $I$. The CKY table together with the $AddedBy$
sets is called a parse-forest, a compact and nice representation of the parse-space (set of
all parse-trees) of the input sentence. A depth-first traversal of the pointers, 
starting at any item \mbox{\ITEM{S}{\alpha}{}$ \in [0, n]$}, leads to retrieving parses
for the input sentence.

A complication, which occurs in implementing a CKY that constructs a parse-forest
in time linear in~$|G|$ is exactly in maintaining the $AddedBy$ sets of binary items. For the item
\ITEM{A}{BC}{}$ \in [i, j]$, there are usually many items \ITEM{C}{\beta}{}$ \in [k, j]$,
for each $i < k < j$ and any $\beta$, that resulted in adding it to the table. Moreover,
usually there are many items \ITEM{C}{\beta}{} in every entry \entry{k}{j} 
that result in adding \ITEM{A}{BC}{} into \entry{i}{j}.
For achieving time-complexity linear in grammar size it is necessary
to maintain for every non-terminal $C$ and for every \entry{k}{j}, \mbox{$i < k < j$},
a set of all items \ITEM{C}{\beta}{}, for any $\beta$ value, in a special set, which
we denote with $Final(C, k, j)$.
Again, this can be achieved only if we implement every entry $[k, j]$ as an array of 
length $|V_{N}|$. At array-entry $C$, of table entry $[i, j]$, we gather 
together all items \ITEM{C}{\beta}{}. Even good hashing-functions can lead to 
sacrificing linearity in grammar-size just because a ``bucket" (in the hash-table) 
containing \ITEM{C}{\beta}{} might
also contain other items \ITEM{D}{\gamma}{}, making the construction of the $AddedBy$ sets,
during {\bf Deduce}, go deep into these buckets in order to filter them. This can lead, 
in the worst case, to time-complexity \mbox{$|G|^{2} \mul n^{3}$}.

The space-complexity of the CKY parser for CFGs is \mbox{$O(|G|^{2} \mul n^{3})$}
(this includes the $O(|G|\mul n^{2})$ recognition and for every item in the recognition
 chart there can be at most $O(|G|\mul n)$ pairs of items in its $AddedBy$ list).
Usually, very efficient storage methods such as bit-vectors can be used
to implement table entries and items, in order to minimize the actual 
memory-consumption for large $|G|$ values. However, these methods have a 
hidden overhead (retrieval time-costs) that might defeat their utility in many 
cases.

For general CFGs, the CKY algorithm has some  known disadvantages:
\begin{itemize}
 \item For many grammars, the transformation of the CFG into CNF 
       results in expanding the grammar dramatically. In some cases,
       the size of the CNF grammar is square the size of the
       original grammar $|G|$~\cite{GrahamEtAl80}. This sets the algorithm
       back at time-complexity proportional to $|G|^{2}$. 
       \cite{GrahamEtAl80} offers solutions for this but in practice, as I argue below, 
       these solutions cannot avoid this problem for very large CFGs.
 \item The characterization of the CKY algorithm given above means that
       an item \ITEM{A}{\alpha}{} is added to \entry{i}{j} regardless of
       whether it participates in a derivation of the string 
       \mbox{$w_{k}^{j} w_{i}^{j} w_{j}^{l}$}, for any \mbox{$0 \leq k < i < j < l \leq n$}.
       Consequently, many of the items added to the table are ``useless" since they do
       not contribute to derivations of the whole input sentence.
       The run-time and memory costs, which these ``useless" items
       imply, can be reduced to a certain degree with simple optimization methods
       discussed also in~\cite{GrahamEtAl80}.
\end{itemize}
Next I argue that, in practice, for real-life DOP STSGs, the above two 
disadvantages imply either very slow speeds or very huge memory costs or both. 
%
\subsection{Computing MPP/MPD for SCFGs}
An algorithm for the computation of the Most Probable Parse (MPP) (and at the same time 
the Most Probable Derivation - MPD) based
on CKY for SCFGs is presented in~\cite{ViterbiCFG,Jelinek}. The computation
does not alter the time or space complexity of the CKY. It is based on
the Viterbi~\cite{ViterbiAlg} observation that two partial-derivations, 
starting from the same root non-terminal $N$ and ending in the same 
portion $w_{i}^{j}$ of the input sentence,
can be extended to derivations of the whole sentence exactly in the same ways. 
Therefore, if the one partial-derivation has a lower probability than the other,
it can be neglected. 

Let be given an SCFG~\SCFG~ and an input sentence $w_{1}^{n}$.
Let \mbox{$MaxP(item, i, j)$} denote the probability of the MPP (MPD) starting
from an item \mbox{$item \in$ \entry{i}{j}}. Figure~\ref{FigMPDCFGs} shows the 
specification of an extension of the CKY algorithm for computing $MaxP$ for
every item in the CKY table. The operator $\sumMPD$ computes the maximum of a set
of reals. The probability of the MPP of the input sentence $w_{1}^{n}$ is then
found as \mbox{$\sumMPD \SETM{MaxP(\ITEMN{S}{\alpha}{}, 0, n)}{\ITEMN{S}{\alpha}{} \in [0, n]}$}.
%
\begin{figure}
\hrule
\begin{tabbing}
$MaxP(\ITEMN{A}{a}{}, i-1, i) = ~P(\RuleM{A}{a})$ \\
\\
$MaxP(\ITEMN{A}{B}{C},$
\= $i, j) =$                                        \\
\> $\sumMPD~ \SETM{MaxP(\ITEMN{B}{\beta}{}, i, j)}{\ITEMN{B}{\beta}{} \in [i, j]}$ \\
\\
$MaxP(\ITEMN{A}{B C}{~},$
\= $i, j) = P(\RuleM{A}{B C}) \mul$        \\
\> $\sumMPD~ \{ MaxP(\ITEMN{C}{\gamma}{}, k, j) ~|~ \exists~ i < k < j, ~\ITEMN{C}{\gamma}{} \in [k, j]$\} \\
\end{tabbing}
\hrule
\caption{The MPD algorithm for CFGs in CNF}
\label{FigMPDCFGs}
\end{figure}
%
Note that in SCFGs a derivation and the parse it generates have exactly the same
probability simply because every parse can be generated by one single derivation.
The algorithm described above can be used for computing the probability of 
the input sentence by replacing every $\sumMPD$ operator with the $\sum$ operator. 
For computing the MPP (MPD) of an input sentence, the algorithm of figure~\ref{FigMPDCFGs}
should be extended with a storage that keeps track of all entities that result in
the maximum value in every $\sumMPD$ term (i.e. replace every $\sumMPD$ by \mbox{$arg max$}). 
%
\subsection{Direct application to DOP STSGs}
\label{SecLargePCFG}
An STSG \STSG~ can be seen as a SCFG, where each elementary-tree
$t$ is considered a production rule ``\Rule{root(t)}{frontier(t)}".
A problem can arise if two internally different elementary-trees result
in the same CFG production rule. To avoid this every elementary-tree
receives a unique address and the address is attached to the rule.
So if the number of elementary-trees in the STSG at hand is denoted by 
\TSGsize, the size of the rule set of the corresponding CFG is also \TSGsize.
Also let $|A|$ denote the number of internal nodes of all elementary-trees
of the STSG. In practice, for real-life DOP STSGs, the number of elementary-trees 
runs in the hundreds of thousands (these figures are obtained on 
limited domain tree-banks such as the OVIS~\cite{DOPNWORep} and 
the ATIS~\cite{HemphilEtAl90}). For future tree-banks and applications,
these numbers are expected to grow. In any case, let us consider what
happens when applying the CKY directly for such huge CFGs that are
obtained from DOP STSGs:
\begin{itemize}
 \item The CFG is not in CNF. As explained earlier,
       a transformation to CNF expands the number of rules and non-terminals
       by the size of that CFG. The size of the CFG, 
       defined above, is the sum of the lengths of its productions. For this
       CFG this is equal to \mbox{\TSGsize $\mul \mu(|rule|)$}, where $\mu(|rule|)$
       is the average length of a rule of the CFG. For linguistic annotations,
       \mbox{\TSGsize $\mul \mu(|rule|)$}
       is of the same order of magnitude as the total number of nodes
       in the DOP STSG's elementary-trees, denoted by $|A|$. 
       In the CKY, to achieve time complexity proportional to linear in $|A|$, 
       each entry of the algorithm must be represented as an array of length $|A|$,
       as the number of non-terminals of the CNF CFG is also in the order of magnitude 
       of $|A|$. In the current limited domain applications the number $|A|$ runs
       also in the hundreds of thousands. Clearly, maintaining such huge entries
       implies such memory-needs that are beyond those that are currently available,
       especially if the application involves large tables for long input sentences or 
       word-graphs (e.g. with up to 70~states).
       Therefore, linearity of the CKY in $|A|$, the STSG size,
       has to be sacrificed and we fall back to $|A|^{2}$ worst case complexity.
       A second issue in CNF transformation is that it may even result in squaring
       the size of the STSG~\cite{GrahamEtAl80}, a thing that also sets us back at the
       $O(|A|^{2} \mul n^{3})$ time-complexity.
 \item The second problem is the huge number of failing derivations in such
       a large grammar. As explained in the preceding section, this implies extra 
       work that leads to useless nodes, useless partial-derivations and useless
       partial-parses.
       Of course this is inevitable in CFG parsing but it is important to minimize its
       effects. Methods that use lookahead variables and rely on knowledge of the 
       grammar can reduce this a bit. But for such a large STSG, this remains a serious
       burdon that begs for an alternative solution.
\end{itemize}
This argues against direct application of the CKY parser for real-life
DOP STSGs. In section~\ref{SecOptAlg} I introduce an algorithm that exploits the
CKY algorithm but avoids these problems. The idea is to first parse with a
very small grammar which approximates the STSGs parse-space. And subsequently to
apply the large STSG on this parse-space in order to conclude the parsing
process with the parse-forest of the STSG.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\section{An optimized algorithm for DOP}
\label{SecOptAlg}
This section presents an alternative to the direct application of the CKY 
algorithm~\cite{CKY} for parsing DOP STSGs. Among the advantages of this alternative
is that this algorithm achieves an almost linear time-complexity 
in STSG-size with substantially less memory costs than the CKY algorithm.

The structure of this section is as follows. Subsection~\ref{SubSecTwoPhase} provides an 
introduction and some necessary definitions. Subsection~\ref{SubSecCNFapprox} describes a simple
approximation of the CNF transformation. Subsection~\ref{SubSecDerRecognition} discusses
the algorithm for recognizing STSG derivations of an input sentence, which constitutes the 
basis for the present optimization algorithm.
Subsection~\ref{SubSecCompMPD} presents the algorithm for 
computing the MPD of an input sentence and explains how with minimal changes it can be adapted 
for computing sentence probability and the MPD of an input parse-tree.
Subsection~\ref{SubSecOptimiz} presents the optimization
that leads to linear time-complexity in grammar-size. And finally, 
subsection~\ref{SecOptAlg4WGs} presents an extension of this optimized algorithm for
disambiguation of word-graphs.
%
\subsection{A two-phase parser}
\label{SubSecTwoPhase}
The algorithm is based on the idea that it is possible to span a good
approximation of the parse-forest of an STSG using a relatively small grammar. 
The exact computation of the STSG's parse-forest takes place on this approximated
parse-forest rather than from scratch. This results in reducing the number of useless 
derivations and the storage costs substantially. Subsequently, a simple optimization,
based on a nice property of sets of paths of STSGs and CFGs, brings the time complexity 
of the two-phase algorithm back to linear in STSG size, without extra 
storage costs.

The small grammar of the first phase is an {\em approximation}\/ of the CNF of the
CFG underlying the given STSG (shortly {\em original CFG}). 
Rather than transforming the elementary-trees
of the STSG into CNF in the usual manner, the transformation is simplified
such that the tree- and string sets of the CNF~CFG, underlying
the CNF~STSG resulting from the transformation,
are supersets of those of the {\em original~CFG}.
This simplified transformation has an advantage over the regular CNF transformation:
the size of the resulting CNF CFG is guaranteed to be of the same order of magnitude 
as that of the original CFG\footnote{Recall that the regular CNF transformation might
expand the number of non-terminals and rules drastically. We discuss this in detail below.}.
Crucially, transforming the STSG elementary-trees to CNF, in the simplified way, 
does not change its (weak and strong) generative power. A suitable correspondence between 
the CNF~CFG rules and the CNF~STSG elementary-trees' nodes allows applying the second 
phase of the parsing algorithm in an efficient manner.
%

Below we need the following definitions:
\begin{description}
\item [String language:] The {\em string-language}\/ of a CFG, SCFG, TSG or STSG $G$,
      denoted ${\cal L}(G)$, is the set of all strings of terminals that it can generate. 
\item [Tree language:] The {\em tree-language}\/ of a CFG, SCFG, TSG or STSG $G$,
      denoted ${\cal T}(G)$, is the set of all parse-trees that it can generate for all
      strings in its string-language.
\end{description}
Moreover, the following property of STSGs plays a central role in our discussion:
\begin{verse}
     {\sl The string/tree language of an STSG is always a subset of the string/tree 
     language of the CFG underlying~it.}
\end{verse}
%
Furthermore, for the rest of this section we assume that we are given a finitely 
ambiguous and $\epsilon$-free STSG $G_{stsg}$, and that the CFG underlying 
$G_{stsg}$, denoted $G_{cfg}$, is also finitely ambiguous and $\epsilon$-free.
%
% [ECNF:]
%  A CFG is said to be in Extended Chomsky Normal Form (ECNF) iff each of its rules
%  is in one of three possible forms: \Rule{A}{a} (terminal form), \Rule{A}{B} (unary form) 
%  or \Rule{A}{B C} (binary form).
%
%  In general it is more convenient to transform CFG to ECNF because,
%  contrary to CNF, it does not erase rules but only expands them. This simplifies
%  the transformation and the transformation back to the original CFG.
%%
\newcommand{\stsg}{$G_{stsg}$}
\newcommand{\cfg}{$G_{cfg}$}
%%%
\subsection{CNF approximation}
\label{SubSecCNFapprox}
The CNF transformation discussed here is a simple approximation of the
well-known CNF transformation of CFGs. Although often the ``traditional" CNF
transformation can also be applied to the CFG underlying the STSG without 
introducing too many rules, I prefer here the following approximation.

The transformation is applied to the elementary-trees of the STSG \stsg. 
Two observations underly this Approximated CNF (ACNF):
%
\begin{itemize}
 \item Every elementary-tree of the STSG is an atomic unit. 
       Every parser must treat the elementary trees as such, in one way or another, 
       in order to compute the parse-forest of the STSG.
 \item Based on the first observation, it does not matter in what way we transform the 
       internal structure of an elementary-tree into CNF, provided that we take care that 
       its atomicity is preserved. In the present parsing algorithm, the second phase takes 
       care of the atomicity of elementary-trees.
\end{itemize}
%
\begin{figure}
\begin{center}
\mbox{
\epsfxsize=125mm
\epsfbox{./D-CH_OptAlg4DOP/D-figures/CNFTrans.eps}
}
\end{center}
\caption{An approximation of the CNF transformation} 
\label{CNFTrans}
\end{figure}
%
Given these two observations, the ACNF transformation starts by assigning to every 
elementary-tree of the STSG a unique address from a domain~$\Pi$.
During the ACNF transformation, every elementary-tree retains its address.
The ACNF transformation has the following steps:
\begin{itemize}
  \item Transform the elementary-trees of \stsg\/ to elementary-trees containing no
        unary productions. 
  \item Transform the elementary-trees, resulting from the preceding transformation,
        to a form where every node, 
        in every elementary-tree, has either children that are all non-terminals 
        or has one single terminal child. 
  \item Transform every resulting elementary-tree to CNF by traversing it
        from its root to its leaves in a breadth-first traversal. Under every
        node in the elementary-tree, encountered during the traversal, there is
        now a production rule; if the production rule is not in CNF then it
        must be a rule $\RuleM{A}{B_{1}\cdots B_{m}}$, where $m > 2$ and all 
        $B_{i}$ is a non-terminal. Transform this rule into a right linear (or left
        linear) structure by introducing exactly $m-2$ nodes labelled 
        with the \underline{same fresh symbol $A^{'}$}. Figure~\ref{CNFTrans} depicts
        this step.
\end{itemize}
The tree- and string-sets of the resulting CNF~CFG are supersets of 
those of the CNF~STSG. In fact, the ACNF transformation results in a CNF~CFG that behaves
in two different ways: 
internal to elementary-trees as a right-linear grammar (a regular grammar) 
and external to elementary-trees as a CFG.

It is important here to restate two simple facts, mentioned above, and sketch their proof 
informally:
%
\newtheorem{CHOptAlgA}{Proposition}[chapter]
\EExample{CHOptAlgA}
{The ACNF transformation results in a CNF~STSG with the same 
string language as the original STSG \stsg. Moreover, up to a simple 
reverse-transformation, the tree language of the CNF~STSG is equal to that
of \stsg.}{CHOptPropA}
%
\DEFINE{Proof~\ref{CHOptPropA}:}
{The transformation alters only the {\em internal
structure}\/ of elementary-trees, i.e. it does not alter the root node or the leaf nodes
and their labels. Exactly the same derivations, substition sequences of elementary-trees
together with their unique addresses, are still possible in the CNF~STSG as the original STSG.
Thus the string language of the CNF~STSG is the same as that of the original STSG.
A simple reverse-transformation gives back the same tree language also. Text books
on parsing exhibit for the first two transformations 
reverse transformations, e.g.~\cite{AHO}. 
For the third step, a reverse transformation simply 
removes every node labeled with $A^{'}$, where $A$ is a non-terminal of the STSG
and uses the unique addresses in order to retrieve the original structures~~$\Box$
}
%
\newtheorem{CHOptAlgB}[CHOptAlgA]{Proposition}
\EExample{CHOptAlgB}
{The string/tree language of the CFG underlying the STSG \stsg, i.e. \cfg,
 is a subset of (respectively) the string/tree language of the CNF~CFG 
 (underlying the CNF~STSG resulting from the approximate CNF transformation).
}{CHOptPropB}
%%
\DEFINE{Proof~\ref{CHOptPropB}:}
{It can be eaily observed that every derivation of \cfg~ is still possible in 
 the ACNF~CFG resulting from the transformation. However, the ACNF~CFG might have extra
 non-terminals introduced during the transformation. This introduces new derivations
 for (possibly) other strings and other trees~~$\Box$
}
%
As mentioned earlier, the string/tree language of an STSG is always a subset of 
(respectively) the string/tree language of the CFG underlying it. Together with the above two
facts this means that the tree/string language of the original STSG is respectively
a subset of the tree/string language of the CNF~CFG. 

The ACNF transformation introduces new rules. The number of the newly introduced
rules is at most equal to the sum of the lengths of the right~hand sides of the rules of
the CFG underlying the STSG, i.e. $O(|G_{cfg}|)$. The number
of non-terminals has grown but it is at most double that of the CFG \cfg.
In this way, we have a small CNF grammar of the same order of magnitude as
the original CFG \cfg. For linguistic CFGs, the right hand sides of rules are 
much shorter than the lengths of frontiers of elementary-trees of DOP STSGs.
And besides, some of the newly introduced rules have more chance to be identical than
in transforming the STSG into CNF, implying even a smaller grammar.
Most importantly, the ACNF transformation, even in the worst-case, does
not result in squaring the size of the CFG.  All in all, this approximation of 
the CNF results in a small grammar that can be parsed very fast using the CKY. 

The transformation results also in a CNF~STSG that has new nodes in its elementary-trees.
As explained above, the number of the new nodes is in the worst case equal to the length
of the frontiers of the elementary-trees, i.e. $O(|A|)$, where $|A|$ is the total
number of nodes in the elementary-trees of the STSG. This doubles the number of nodes
in the worst-case, but the CNF approximation introduces only $O(|G_{cfg}|)$ new
non-terminals (as opposed to $O(|A|)$ in the usual CNF transformation, as explained earlier). 
%
%%%%%%%%%%%%%%%%%%%%%
\subsection{STSG-derivations recognition}
\label{SubSecDerRecognition}
Be given an STSG \stsg\/ $=$ \STSG~ in CNF (the transformation to CNF is as
described above). The input sentence is denoted $w_{0}^{n}$, where 
\mbox{$w_{0} = \epsilon$}. The present algorithm has the structure:
%
\begin{enumerate}
 \item [Phase 1.] Apply the CKY algorithm using the (CNF) CFG underlying
                  \stsg, denoted \cfg, resulting in a parse-forest of the input sentence.
                  As mentioned above, this parse-forest is a superset of the parse-forest
                  which \stsg\/ spans for the same sentence.
 \item [Phase 2.] Apply an algorithm, described below, for computing the parse-forest 
                  of \stsg\/ {\em from the approximate parse-forest}\/ of the previous phase,
                  and compute the MPD on this parse-forest.
                 % Apply the reverse-transformation, mentioned above, to the resulting MPD.
\end{enumerate}
Often, I will refer to the first phase with the general term ``parsing phase" 
and to the second phase with the term ``disambiguation-phase". Both terms do not 
reflect the exact task of each phase. They only reflect the main task of each
phase: (approximating) parse-forest generation in the first, and  
computation of the MPD, i.e. the selection of one preferred tree from the exact
parse-forest, in the second.

Below I discuss the second phase, which fulfils three requirements: preserve 
atomicity of \stsg's elementary-trees, preserve the uniqueness of every 
elementary-tree, and recognize exactly \stsg's parse-forest and derivations for
the input sentence from the CFG parse-forest. But first I discuss the issue of how to 
recognize a derivation of \stsg~ when given a parse-forest of \cfg.
The issue of recognizing an STSG derivation is central in the MPD-computation 
algorithm. But first the following definitions.
%
\DEFINE{Node address:}
{This is a unique address from some domain $\Pi$ assigned to a non-leaf node in an 
 elementary-tree of \stsg. 
}
Every non-leaf node in every elementary-tree of \stsg is assigned such a unique node-address 
from $\Pi$. It is useful if the addresses of the nodes of an elementary-tree enable fast 
checking of the parent-child (and the number of the child if counting from left to right)
and sisterhood relations between nodes in an elementary-tree. 
%
\DEFINE{Decorated tree:}
{A tree in which every non-leaf node is {\em decorated}\/ with exactly one address, from the
 STSG elementary-trees' node addresses, is called a decorated tree. The collection of
 node addresses in a decorated tree is called the {\em decoration} of that tree.
}
%
\DEFINE{Derivation-tree:}{Every derivation of the STSG can be characterized by a
          unique decoration of the tree it generates; in this decoration every node 
          in the tree is decorated with the unique address of the corresponding node
          of an elementary-tree. We refer to this decorated tree with the term 
          {\em derivation-tree}. 
}
%
\begin{figure}[tbh]
\hrule
\begin{tabular}{c}
\epsfxsize=90mm
\epsfbox{./D-CH_OptAlg4DOP/D-figures/ExplViab.eps} \\
\\
\\
\epsfxsize=130mm
\epsfbox{./D-CH_OptAlg4DOP/D-figures/Viabi.eps} 
\end{tabular}
\hrule
\caption{(Top) decorated tree, (bottom) the viability property}
\label{FigViab}
\end{figure}
%
%
Note that not every decorated tree is a derivation-tree since some decorations
do not correspond to STSG derivations. We observe that a simple algorithm can be 
used for recognizing whether a decorated tree is a derivation-tree of \stsg\/ or not. 
To this end, we need to define the {\em viability property}, a main element of this
algorithm and the algorithm for computing the MPD.
%
\DEFINE{Viability property:}
{Let $X$ be a node in a decorated-tree, labeled $N$ and decorated with address $c$, 
 and let $Xch$ be its $j$th child-node, labeled $N_{j}$ and decorated 
 with address $c^{'}$, $j \in \{1,2\}$. We say that the viability property holds for 
 nodes $X$ and $Xch$ if one of the following two holds (see figure~\ref{FigViab}):
 \begin{description}
  \item [Parenthood:] There is some elementary-tree, in \stsg, for which 
       $c$ and $c^{'}$ correspond to two of its non-leaf nodes that are related (respectively)
       as parent and its $j$th child. Moreover the node corresponding to $c$/$c^{'}$ 
       in that elementary-tree is labeled respectively with $N$/$N_{j}$.
  \item [Substitution:] 
        There is some elementary-tree, in \stsg, for which the address $c$ corresponds 
        to one of its nodes that is labeled $N$ and that has a leaf child-node labeled 
        with a non-terminal $N_{j}$, i.e. a substitution-site.
        And there is some elementary-tree, in \stsg, for which the
        address $c^{'}$ corresponds to its root node that is labeled $N_{j}$. 
 \end{description}
}
%
The algorithm for recognizing whether a decorated tree is a derivation-tree of \stsg\/ 
is shown is figure~\ref{AlgRecDerT}; we will refer to it with the name 
algorithm~\ref{AlgRecDerT}. 
%
\begin{figure}[h]
\hrule
\vspace*{.3cm}
\begin{description}
  \item [Root:] Check whether the root of the tree is labeled $S$ and is decorated with
    an address which corresponds to the root of an elementary-tree.
    If not then goto {\bf Fail} below.
  \item [Iterate:] For every node in the decorated tree, that is not a leaf node, do:\\
          {\bf 1)}~let that node be the current node, \\
          {\bf 2)}~for the current node $X$, labeled $N$ and decorated 
         with address $c$, and its $j$th child-node $Xch$, labeled $N_{j}$ and decorated 
         with address $c^{'}$, $j \in \{1,2\}$, check that the viability property 
         holds for $X$ and $Xch$, otherwise goto {\bf Fail}.
%  \begin{description}
%   \item [\underline{Viability property}] 
%   One of the following two must hold (figure~\ref{FigViab}):
%  \begin{description}
%   \item [Parenthood:] There is some elementary-tree, in \stsg, for which 
%       $c$ and $c^{'}$ correspond to two of its non-leaf nodes that are related (respectively)
%       as parent and its $j$th child. Moreover the node corresponding to $c$/$c^{'}$ 
%       in that elementary-tree is labeled respectively with $N$/$N_{j}$.
%   \item [Substitution:] 
%        There is some elementary-tree, in \stsg, for which the address $c$ corresponds 
%        to one of its nodes that is labeled $N$ and that has a leaf child-node labeled 
%        with a non-terminal $N_{j}$, i.e. a substitution-site.
%        And there is some elementary-tree, in \stsg, for which the
%        address $c^{'}$ corresponds to its root node that is labeled $N_{j}$. 
%  \end{description}
%  \end{description}
  \item [Accept:] return accept and exit.
  \item [Fail:] return reject and exit.
\end{description}
\hrule
\caption{Algorithm~\ref{AlgRecDerT}: Recognizing a derivation-tree}
\label{AlgRecDerT}
\end{figure}
%

%
The following propositions express the role which the viability property plays 
in recognizing derivation-trees.
%
\newtheorem{CHOptAlgBB}[CHOptAlgA]{Proposition}
\EExample{CHOptAlgBB}
{If a decorated tree contains a node that does not fulfill the viability property,
 the decorated tree is not a derivation-tree of the STSG at hand.
}{CHOptPropBB}
%
\newtheorem{CHOptAlgBA}[CHOptAlgA]{Proposition}
\EExample{CHOptAlgBA}
{Algorithm~\ref{AlgRecDerT} recognizes a decorated tree 
 iff it is a derivation-tree of the STSG at hand. 
}{CHOptPropBA}
%
The proofs of these two propositions are simple to construct 
and will be skipped here. 

%
As a result to the propositions above, if given a parse-forest, spanned by 
the STSG \stsg\/ for some input sentence, it is possible to determine the set 
of all derivation-trees of the sentence by applying the above algorithm to the 
parse-forest. However, applying this algorithm
blindly would result in exponential time-complexity. It is necessary to apply it
in an efficient manner. Moreover, instead of applying the recognition of the
derivation-trees of a sentence to \stsg's parse-forest, we may apply it to the
CFG's parse-forest; this determines the derivation-trees of the sentence according
to the STSG \stsg\/ and, as a side effect, this delimits \stsg's parse-forest for
the sentence, since trees without \stsg's derivation-trees are not trees of \stsg. 

To obtain a (deterministic) polynomial-time algorithm for the recognition of the set
of derivation-trees of an input sentence, we employ a new compact structure, in analogy
to a parse-forest, called a {\em derivation-forest}\/ of the sentence. To this end, define:
%
\DEFINE{Rule occurrence:}
{Let rule \mbox{$R \in$ \Rules} be found under a non-leaf node with address $c$ of a given 
 elementary-tree. The address $c$ is called an occurrence of $R$ in that elementary-tree.
 An occurrence of an item \ITEM{A}{\alpha}{\beta} is an occurrence of the rule
 $\RuleM{A}{\alpha\beta}$.
}
%
\DEFINE{Occurrence set:}{
 The {\em occurrence set}, denoted $\An(R)$, of a given rule \mbox{$R \in$ \Rules}
 is the set of all occurrences of $R$ in all elementary-trees of \stsg.
% The occurrence set of an item is equal to the occurrence set of the rule underlying
% that item.
}
%
\DEFINE{Item's occurrences set:}
{Let \ITEM{A}{\alpha}{\beta} $\in$ \entry{i}{j}. The {\em occurrences set}\/
of this item is defined as 
 $\An(\ITEMN{A}{\alpha}{\beta},~i,~j)$ = $\An(\RuleM{A}{\alpha\beta})$.
}
%
Given the CFG parse-forest and the CKY table of the input sentence, built by the CKY algorithm,
a decoration of the items in the table enables recognizing the derivation-forest
of that sentence. We maintain with every item its occurrence set.
The derivation-forest is constructed on top of the CFG parse-forest, also in a 
bottom-up fashion by applying an algorithm for recognizing derivation-trees to the 
occurrence sets of the items that are connected together in the parse-forest 
by the $AddedBy$ relation described in the previous section. 
Similar to our presentation of the Viterbi CKY, we do not show exactly how 
to construct the derivation-forest, instead we show how to compute the MPD of the input
sentence. The construction of the derivation-forest extends the MPD algorithm described
below only by associating sets of pointers between occurrences of items. Recall that
if an item $B$ results in adding another item $A$ to entry \entry{i}{j}, during {\bf Deduce}
of CKY, then  $B \in AddedBySet_{A, i, j}$, where this expresses a pointer from $A$ to
$B$. Similarly, a set is associated with every occurrence, $c$, of $A$, denoted 
$ViabilitySet_{c,A}$. If $B \in AddedBySet_{A, i, j}$ and $b$ is an occurrence of $B$,
then $b \in ViabilitySet_{c, A}$ iff a predicate $Viable?(c, b, j)$, 
defined below, is true; except for final binary items, $j$ is always equal to 1.
For final binary items, the value $j \in \{1, 2\}$ allows testing the predicate 
$Viable?(c, b, j)$ for the left (``first child")  or right (``second child") 
items in the pairs of items in $AddedBy$ of the final binary item.
The predicate $Viable?$ tests the viability property defined earlier for 
the algorithm~\ref{AlgRecDerT} for recognizing derivation-trees. 

%------- now we are ready to do the data structures and present the algorithm !!
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computing the MPD}
\label{SubSecCompMPD}
For computing the MPD of an input sentence under \stsg, it is useful to precompile
the \stsg\/ into a form that makes the viability property explicit. 
To this end, infer the following predicates and functions from \mbox{\stsg $=$ \STSG}:
\begin{enumerate} 
\item {\bf $Parent?(c,~c^{'},~j)$} denotes the proposition 
      ``{\em $c$ and $c^{'}$ 
      are the addresses of a parent and its $j$-th child in an elementary-tree in \Corp}".
\item {\bf $Root?(c)$} denotes the proposition 
      ``{\em $c$ is the address of the root node of an elementary-tree in \Corp}".
\item {\bf $TreeOf(c)$} denotes the function that returns $t \in $\Corp
       such that $c$ is the address of some node in $t$. 
%\item {\bf $TreeOf(c)$} denotes the function ``if $Root?(c)$ is true then return 
%       the (identity or address) of the elementary-tree, which has $c$ as address 
%       of its root, else return null".
\item {\bf $SubSite?(c,j)$} denotes the proposition ``{\em child nr. $j$ 
       of the node with address $c$, in some elementary-tree,
        is a substitution-site}\/".
\end{enumerate} 
%
\newcommand{\BULLET}{\hspace*{-.5cm}$\bullet$~}
\newcommand{\hspx}{\hspace*{-.6em}}
Then infer the eight-tuple \RBSTSG, from \stsg, where:\\
%
\begin{tabular}{rcl}
\\
\multicolumn{3}{l}{
\BULLET \CFG~ is the CFG underlying~\STSG,}     \\
\\
%\multicolumn{3}{l}{
\BULLET
$\forall$ $R \in \RulesN$: ~${\cal A}(R)$ & =  &
$\{c~| c$ is the address of an occurrence of $R \},$
\\ %}\\
\\
\multicolumn{3}{l}{
\BULLET
$Viable?(c,~c_{j},~j)$  ~=~ 
          $Parent?(c, c_{j}, j)$ ~\OR~ $(~ SubSite?(c, j)$ ~\AND~ $Root?(c_{j})~)$,
} \\
\\
%\multicolumn{3}{l}{
{\bf \A} & = & \SET{\A$(R)$}{$R \in$ \Rules},
\\ %}\\
\\
\multicolumn{3}{l}{
\BULLET
$P$ : $\Pi$ \lra $(\Pi\multi\{1, 2\})$ \lra $[0..1]$,
}\\
\multicolumn{3}{l}{
For $c, c^{'}\in\Pi$ and $j\in\{1, 2\}$: 
}\\
\multicolumn{3}{l}{
\hspace*{-.4cm}
\begin{tabular}{lll}
 $P(c)(c^{'},j)$ & = & $\left\{
        \begin{tabular}{ll}
       \hspx $PT( TreeOf(c) )$ & [$j=2$ \AND~ $Viable?(c, c^{'}, j)$ \AND~ $Root?(c)$] \\
       \hspx {\bf 1} & [$Viable?(c, c^{'}, j)$ \AND~ ($j=1$ \OR~ {\bf not} $Root?(c)$)] \\
       \hspx {\bf 0} & [\bOtherwise],\\
        \end{tabular}
        \right.$
\end{tabular}
}\\
\\
\multicolumn{3}{l}{
\BULLET
$PF$ : $\Pi$ \lra $[0..1]$,}\\
\multicolumn{3}{l}{for $c \in \Pi$:  }\\
\multicolumn{3}{l}{
\begin{tabular}{lll}
 $PF(c)$ & = & $\left\{
        \begin{tabular}{ll}
          $PT( TreeOf(t) )$ & [$Root?(c)$] \\
          {\bf 1} & [~{\bf not} $Root?(c)$] \\
        \end{tabular}
        \right.$
\end{tabular}
}\\
\\
\end{tabular}
%

The predicate $Viable?()$ formalizes the viability property.
For a decorated tree, in which $c$ decorates a node $X$, 
the term $P(c)$ denotes the probability of $c$~as a function of 
the address $c^{'}$ of the $j$th child of $X$ (counting children is always from left
to right).This definition enables writing the algorithm as a recursive function.
$P$ expresses the probabilities in terms of the ``probabilities" of the rules 
of the CFG underlying \stsg; the probability of a rule of the CFG underlying 
\stsg\/ is a function of its particular occurrence, i.e. address, in the 
elementary-trees set of \stsg. 

\begin{figure}[thb]
\hrule
\[
\begin{array}{rl}
&  \\
P_{mpd}(w_{0}^{n}) \hspf  \hspf = & 
\sumMPD_{\tiny\hspf\TABS
{\ITEM{S}{\alpha}{}$\in \entryN{0}{n}$} 
{$c\in \An(\ITEMN{S}{\alpha}{},~0,~n)$}
{and $Root?(c)$}{}}
Pp(c,~\ITEMN{S}{\alpha}{},~0,~n)\\
\mbox{ }  & \\
%\hspfth
Pp(c,item,i,j) \hspf =\hspf  &  \hspf \bCase item~\bOf \\
\mbox{ }  & \\
\hspfth
\ITEMN{A}{w_{i+1}}{} \hspft \hspfth :\hspfth & \hspfth PF(c),~~~$where$ ~$j = i+1$,  \\
\\
\hspfth
\ITEMN{A}{B}{C} \hspft \hspfth :\hspfth &  \hspfth
  \overbrace{
       \STACK{\sumMPD}{\alpha}
       \STACK{\sumMPD}{c1\in \An(\ITEMN{B}{\alpha}{},i,j)}
        P(c)(c1, 1)\mul
        Pp(c1, \ITEMN{B}{\alpha}{}, i, j)}, \\
\\
\hspfth
\ITEMNM{A}{BC}{} \hspft \hspfth :\hspfth& \hspfth
\sumMPD_{i < k < j}~Pp(c, \ITEMN{A}{B}{C}, i, k)~\mul \\
 & 
        \overbrace{
       \sumMPD_{\alpha}
            \sumMPD_{c2\in \An(\ITEMN{C}{\alpha}{}, k, j)}
P(c)(c2, 2)\mul Pp(c2, \ITEMN{C}{\alpha}{}, k, j)}
\end{array}
\]
\caption{Algorithm~\ref{AlgPS} for computing the MPD of a sentence $w_{0}^{n}$}
\label{AlgPS}
\vspace{1em}
\hrule
\end{figure}

Let $\sumMPD_{Pred(x)}A(x)$ denote the maximum of the set \mbox{\{$A(x)$~/~ $Pred(x)$\}}.
The algorithm for computing the MPD of a sentence $w_{1}^{n}$ 
is shown in figure~\ref{AlgPS}, also referred to as algorithm~\ref{AlgPS}. 
It computes the MPD of the input sentence 
on the parse-forest, which was constructed in the first phase by the CKY of the CFG \cfg.
The function $P_{mpd}(w_{0}^{n})$ computes the 
probability of the MPD of the sentence $w_{0}^{n}$, where \mbox{$w_{0} = \epsilon$}. 
The function $Pp:~\Pi\multi~ITEMS\multi~[0,~n]\multi~[0,~n]\rightarrow~[0,~1]$ 
computes recursively the probability of the most probable among the 
``partial-derivations"\footnote{
Below we define formally the probability of a partial derivation-tree, a more
suitable term, in this context, than partial-derivation.
},
that start with address $c$ and generate a partial-tree for $w_{i}^{j}$. 
%

Note that for SCFGs, i.e. when the elementary-trees of \stsg have no internal nodes, 
the algorithm in figure~\ref{AlgPS} computes the MPD exactly as 
algorithm~\ref{FigMPDCFGs}. This becomes more obvious if one notices that
the probability function $P(c)$ always computes to $PT(t)$ or $1$, due to the fact that
the elementary-trees have no internal nodes at all. For the general case of 
STSGs, a proposition and its proof, following the next definitions, take 
care of the correctness of the present algorithm. 
%
\DEFINE{Partial derivation-tree:}
{A {\em partial derivation-tree}\/ of an STSG is a partial-tree,
 resulting from a partial-derivation of the CFG underlying that STSG, in which
 each node is decorated with a node-address such that {\em the viability property
 still holds}\/ for each of the nodes.
}
%
A partial derivation-tree consists of, on the one hand, a sequence 
of elementary-tree substitutions, and on the other hand, other ``pieces" of elementary-trees.
A piece is a decorated subtree, of an elementary-tree, that either contains the root or 
some leaf-nodes of that elementary-tree but not both. The elementary-trees and the pieces
in the partial derivation-tree are combined with substitution under the STSG's 
viability property, i.e. substitution is allowed only of a node that 
has the address of a root of an elementary-tree on a node that originally was a
substitution-site in an elementary-tree. 

We will say that an elementary-tree {\em fully}\/ participates in a partial derivation-tree
$DT$ iff the addresses of all its nodes decorate nodes in $DT$. And we will say that an 
elementary-tree {\em partially}\/ participates in a partial derivation-tree $DT$ iff the
addresses of some of its nodes do not decorate a node in $DT$, but the addresses of
the other nodes do decorate nodes in $DT$.
%
\DEFINE{Sub-derivation:}
{For every partial derivation-tree there is exactly one corresponding sequence of 
 substitutions, of both the elementary-trees that fully and those that partially participate 
 in that partial derivation-tree;
 this sequence is denoted with the term the {\em sub-derivation} corresponding to the
 partial derivation-tree. 
}
%
In particular, a derivation of the STSG is a sub-derivation 1)~that starts with an 
elementary-tree with a root node labeled $S$, 2)~that has leaf nodes labeled with
terminals and 3)~in which every elementary-tree fully participates.
%
\DEFINE{Probability of a sub-derivation:}
{The probability $Pp(DT)$ of a sub-derivation $DT$ is equal to the 
 multiplication of the probabilities of all elementary-trees that {\em fully}\/ 
 participate in it. 
 The probability of a partial derivation-tree is equal to the probability of the 
 corresponding sub-derivation.
}
%%
%
%
Thus, a partial derivation-tree corresponds to some ``acceptable" 
decoration of a partial-tree's nodes. The viability property determines the ``acceptable"
decorations that corresponds to actual sub-derivations of the given STSG.
The algorithm in figure~\ref{AlgPS}, in short algorithm~\ref{AlgPS},
exploits the viability property by assigning zero to non-acceptable decorations 
and the right probability to the acceptable decorations. 

%
%%%%%%%%%
%Proof of correctness:
%
%%%%%%%%
\newtheorem{CHOptAlgC}[CHOptAlgA]{Proposition}
\EExample{CHOptAlgC}
{$\forall~ item \in$ \entry{i}{j}, $0 \leq i < j \leq n$, and
\mbox{$\forall ~c \in \An(item, i, j)$}, $Pp$~fulfills one of two:
   \begin{itemize}
    \item \mbox{$Pp(c, item, i, j)$,} is equal to the maximum probability of 
     all possible partial derivation-trees $dt$ of $w_{i}^{j}$, 
     that fulfill
     \begin{itemize}
      \item if $item = $\ITEM{A}{\alpha}{} then
         $dt$ has a root node labeled $A$, decorated with $c$, 
         and has children labels that (when concatenated from left to right) 
         form a string equivalent to $\alpha$, 
      \item if $item = $\ITEM{A}{B}{C} then
         $dt$ has a root node labeled $B$ and decorated with $c^{'}$ such that
         $Viable?(c, c^{'}, 1)$ is true.
     \end{itemize}
    \item There are no such partial derivation-trees as in the preceding case
          and \mbox{$Pp(c, item, i, j)$} is equal to zero. 
    \end{itemize}
}{CHOptPropC}
%
\DEFINE{Proof~\ref{CHOptPropC}:}
{The proof is by induction on $x$, $1 \leq x = (j-i) < n$. It depends partially on the CKY 
  property that $\ITEMN{A}{\alpha}{\beta} \in [i,j]$ {\bf iff}
  \mbox{$\RuleM{A}{\alpha\beta}$ \lmdir $w_{i}^{j}\beta$}.
\begin{description}
 \item [${\bf x = 1:}$] Then $\alpha = w_{i+1}$. 
   By the CKY property, there is at most one partial derivation-tree possible in this case, 
   i.e. $\RuleM{A}{w_{i+1}} \in \RulesN$ with $A$ decorated with $c$. 
   Therefore, $Pp(c, \ITEMN{A}{w_{i+1}}{}, i, i+1) = PF(c)$. The proposition holds since
   there is only one partial-derivation tree.
%
 \item [${\bf x = m:}$] Assume the proposition holds for all $1 \leq x \leq m$, $m < n$.
 \item [${\bf x = m+1:}$] Let \ITEM{A}{\alpha \beta}{} $\in$ \entry{i}{j} and 
                  $c \in \An(\RuleM{A}{\alpha\beta})$.
                  By the CKY property there is a partial CFG-derivation (or many such derivations)
                  \mbox{$\RuleM{A}{\alpha\beta}$ \lmdir $w_{i}^{j}\beta$}.
                  Now there are two cases:
     \begin{description}
      \item [\underline{$\alpha = B C, \beta = \epsilon$:}]
                     Again by the CKY property, for every partial CFG-derivation,
                    \mbox{$\RuleM{A}{B C}$ \lmdir $w_{i}^{j}$}, there 
                    is $i < k < j$ such that there are two 
                    partial CFG-derivations: 
                    \mbox{$\RuleM{A}{B C}$ \lmdir $w_{i}^{k} C$} and
                    \mbox{$C$ \lmdir $w_{k}^{j}$}.
                    The proof now is for every  $i < k < j$ for which this is true.
                    For the current value of $k$, let us consider the probabilities of
                    the possible decorations, of the partial CFG-derivation of $w_{i}^{j}$
                    at hand, that have $c$ decorating $A$ in \ITEM{A}{B C}{}.
                    As explained above, with every such decoration there are (at least) 
                    two decorated partial CFG-derivations for $w_{i}^{k}$ and $w_{k}^{j}$.
                    By the CKY property and the inductive assumption three things hold for these
                    pairs of decorations:
                    \begin{enumerate}
                      \item [a.] 
                       for all $\gamma$, for all $cb \in \An(\RuleM{B}{\gamma})$,
                       \mbox{$Pp(cb, \ITEMN{B}{\gamma}{}, i, k)$}
                       is equal either to zero or to the maximum probability of all partial
                       derivation-trees of $w_{i}^{k}$ starting at 
                       $\RuleM{B}{\gamma}$ with $B$ decorated with address $cb$. 
                      \item [b.] 
                       \mbox{$Pp(c, \ITEMN{A}{B}{C}, i, k)$}
                       is equal either  to zero or to the maximum probability of any partial
                       derivation-tree of $w_{i}^{k}$
                       starting at $\RuleM{B}{\gamma}$ with $B$ decorated with address $cb$ and
                       $Viable?(c, cb, 1)$ is true. 
                      \item [c.] 
                      for all $\delta$, for all $cc \in \An(\RuleM{C}{\delta})$,
                      \mbox{$Pp(cc, \ITEMN{C}{\delta}{}, k, j)$}
                      is equal either to zero or to the maximum probability of any partial
                      derivation of $w_{k}^{j}$
                      starting at $\RuleM{C}{\delta}$ with $C$ decorated with address $cc$. 
                    \end{enumerate}
                     If \mbox{$Pp(c, \ITEMN{A}{B}{C}, i, k)$} is zero for the current value
                     of $k$, then $Pp(c, \ITEMN{A}{B C}{}, i, j)$ is also zero. By the
                     inductive assumption we conclude that there is no partial derivation-tree
                     starting at \ITEM{A}{B C}{} and where $A$ is decorated with $c$, for the
                     current value of $k$. If it is not zero, we face two cases
                     for all $\delta$ and for all $cc \in \An(\RuleM{C}{\delta})$:
                    \begin{enumerate}
                     \item $Viable?(c, cc, 2)$ is false: then $P(c)(cc, 2) = 0$
                     \item $Viable?(c, cc, 2)$ is true: 
                            $P(c)(cc, 2)$ is either $PT( TreeOf(c) )$ or $1$, depending on
                             whether $Root?(c)$ is true or not.
                    \end{enumerate}
                     The last case in the switch of algorithm~\ref{AlgPS} 
                     (case \ITEM{A}{BC}{}) takes the maximum of all
                     $P(c)(cc,2) \mul Pp(cc, \ITEMN{C}{\delta}{}, k, j)$,
                     for all $\delta$ and for all $cc \in \An(\RuleM{C}{\delta})$.
                     By the inductive assumption and the viability property and the definition
                     of partial derivation-trees, this is equal  either to zero or to
                     the maximum probability of all partial derivation-trees starting at
                     \ITEM{A}{B C}{} with address $c$, for this value of $k$.
                     Again by the inductive assumption, multiplying this with 
                     $Pp(c, \ITEMN{A}{B}{C}{}, i, k)$ and maximizing this for all values of
                     $k$ proves the proposition for this case.
%
      \item [\underline{$\alpha = B, \beta = C$:}]
        The proof for this case follows a similar line of argumentation 
        as the preceding case.~~~~$\Box$
      \end{description}
 \end{description}
}
%%%%
\newtheorem{CHOptAlgD}[CHOptAlgA]{Proposition}
\EExample{CHOptAlgD}
{Algorithm~\ref{AlgPS} computes the MPD of $w_{1}^{n}$ under \stsg.
}{CHOptPropD}
%
\DEFINE{Proof~\ref{CHOptPropD}:}
{Easy to derive from algorithm~\ref{AlgPS}, proposition~\ref{CHOptPropC} and
 the unique correspondence between derivation-trees and STSG derivations.~~~$\Box$
}
%%
%
%Complexity analysis
\paragraph{Complexity:}
The time complexity of the second phase of the algorithm is \mbox{$O(|\An|^{2} \mul n^{3})$}.
And the time complexity of the first phase is $O(|\RulesN| \mul n^{3})$. 
For DOP STSGs $|\RulesN|$, the size of the CFG underlying the STSG, is usually 
in the order of $1\%$ of $|\An|$. Therefore in practice the algorithm given above
behaves as if having time-complexity \mbox{$O(|\An|^{2} \mul n^{3})$}.
However, a simple optimization, discussed below, reduces the time-complexity of
the second phase to \mbox{$O(|\An| \mul n^{3})$}.
Moreover, the algorithm computes the second phase on the result of the first phase, i.e.
a parse-forest that already pruned many of the failing STSG derivations. This 
saves space and time that are expected to be much larger than the small overhead of 
having a first and a second phase. The net effect is faster computation that 
uses smaller space. 
%

%Discuss probab of a sentence algorithm
%Discuss probab of a tree algorithm
\paragraph{Derived algorithms:}
Algorithm~\ref{AlgPS} can be easily modified to result in other useful algorithms.
To compute the probability of the input sentence, as the sum of the probabilities of 
all its derivations, exchange $\sumMPD$ with the operator $\sum$ everywhere in the
specification of the algorithm. For computing the MPD and the probability of a given 
parse-tree, the first phase of the algorithm is exchanged for a small algorithm that
transforms the parse-tree into a CKY table with items in the entries; the second phase
is applied as is either with $\sumMPD$ or with $\sum$, depending on the algorithm wanted.

\paragraph{Implementation issues:}
%Issues of implementation: 1. follow the CFG parse-forest 2. failing derivations die
It is important to note that, for clarity of presentation, the specification given in 
figure~\ref{AlgPS} is not as efficient as the algorithm can be implemented.
For implementing the second phase of the algorithm, one precompiles the STSG, as explained
above, in order to make the viability property tables explicit.
The second phase is applied on the parse-forest in a bottom-up fashion
(rather than top-down recursion as the specification does)
making use of the $AddedBy$ sets of the items in the parse-forest
of the first-phase. Moreover, failing sub-derivations, which have probability zero, 
are neglected (rather than dragged together with the others all the way).
%
%%%%%%%%%%%%%5
\subsection{Optimization: approaching linearity in STSG size}
\label{SubSecOptimiz}
% The optimization of the TSG MPD computation.
%
%Due to a property of 
Here we discuss an important optimization of algorithm~\ref{AlgPS}, based on
the following property of STSGs:
%
\DEFINE{Paths:}{ A sequence of nodes, i.e. pairs of labels and addresses, starting at the root 
          node of a derivation-tree and terminating at a leaf node (labeled with a terminal
          symbol) is called a {\em path}\/ of the derivation-tree.
}
%
\DEFINE{Path set:}{ The {\em path set}\/ of a derivation-tree is the set of all paths
           in that derivation-tree. The path set of a given {\em tree}\/ is the union of the
           path sets of all derivations that generate the tree under the STSG at hand. 
           Similarly, the path set of a {\em sentence}\/ is the union of all path sets of the  
           derivations that generate it under the STSG at hand. The path set of the
           STSG is the union of the path sets of the sentences in its string language.
}
%
\begin{description}
  \item [{\bf Relevant property:}] The path set of an input sentence under a TSG is a
          regular language. This property is known to be true for CFGs~\cite{Thatcher71}
          and can be easily proved for TSGs.
\end{description}
%
This property implies that recognition of the path set, and also the derivations, of
an input sentence under an STSG should be possible in time complexity linear in the
number of possible node-labels and their addresses, i.e. $|\An|$. 
A simple observation, related to the viability property,
makes this even clearer: in an elementary-tree, a node labeled $A$ with address $c$
can be only in one of the following two configurations:
\begin{itemize}
 \item $SubSite?(c, j)$ is true, i.e.\ the $j$th child of $c$ is a substitution-site in
       the elementary-tree (i.e.\ a frontier non-terminal). In this configuration, \linebreak
       \mbox{$Viable?(c, cj, j)$} is true only for all $cj$ such that $Root?(cj)$.
 \item $Parent?(c, cj, j)$ is true for some $cj$, i.e. $c$ and $cj$ are both internal to 
          the elementary-tree and are respectively the addresses of a parent and its 
          $j$th child in that elementary-tree. Only one single $cj$ fulfills this (due
          to the unique addresses of nodes in elementary-trees).
\end{itemize}
%
Let $itemP$ denote any item to the left of the semicolon in algorithm~\ref{AlgPS}.
And let $itemCh$ denote any item found in the overbraced term also in 
algorithm~\ref{AlgPS}. The algorithm checks the viability of every
address $c \in \An(itemP)$ with address $cj \in \An(itemCh)$. The above observation says
that this is unnecessary since there are only two complementary configurations in which
$c$ and $cj$ fulfill the viability property. In fact it says even that $c \in \An(itemP)$ 
can be in one of two configurations, and $cj \in \An(itemCh)$ can also be in one of two 
{\em corresponding}\/ configurations.  This motivates partitioning $\An(itemP)$
and $\An(itemCh)$ into:
%
 \begin{eqnarray*}
 HasSubSite(itemP, j) & = & \{c \in \An(itemP)~|~SubSite?(c, j) ~is~true \},\\
 HasChild(itemP,j) & = &  \An(itemP)~-~HasSubSite(itemP, j), \\
 & & \\
 RootsOf(itemCh) & = & \{cj \in \An(itemCh)~|~Root?(cj)  ~is~true \}, \\
 InternOf(itemCh) & = & \An(itemCh)~-~RootsOf(itemCh) \\
 \end{eqnarray*}
%
Recall that the viability property states that:
\begin{verse}
$Viable?(c, cj, j)$ is true for $c \in \An(itemP)$ and $cj \in \An(itemCh)$ iff
either [$c \in HasSubSite(itemP, j)$ and  $cj \in RootsOf(itemCh)$]
or [$c \in HasChild(itemP, j)$ and $cj \in InternOf(itemCh)$].
\end{verse}
The above mentioned observation extends it and states that:
\begin{verse}
For \underline{every} $c \in HasSubSite(itemP, j)$ and \underline{every}
$cj \in RootsOf(itemCh)$ holds $Viable?(c, cj, j)$ is true. 
And, for every $c \in HasChild(itemP, j)$, there is
\underline{at most one} $cj \in InternOf(itemCh)$ such that $Viable?(c, cj, j)$ is true.
\end{verse}
%%
For both cases it is possible to conduct the computation for every $c \in itemP$ in
$O(1)$ rather than $O(|\An|)$ (i.e. $|\An(itemCh|)$). In the first case, 
compute only once the set $RootsOf(itemCh)$ and its maximum probability and pass this
to {\em every}\/ $c \in HasSubSite(itemP, j)$. 
In the second case, an off line  precompilation of 
the place of the $j$th child, for $j \in \{1, 2\}$, of every $c \in HasChild(itemP, j)$ in
$\An(R)$, for every $R$ enables finding it in $O(1)$; then the maximum probability of the
$j$th child is passed to $c$ for computing its maximum probability in $O(1)$.

More formally, the overbraced expression in figure~\ref{AlgPS} in each of the 
last two cases of algorithm~\ref{AlgPS} is rewritten. Let these two expressions 
be denoted by the more general expression
%
\[\STACK{\sumMPD}
        {\alpha,~c_{l}\in \An(itemCh,m,q)} P(c)(c_{l}, l)\mul Pp(c_{l}, itemCh, m, q). \]
%
Substitute for this expression the following,
where $item, i$ and $j$ are as defined by algorithm~\ref{AlgPS}:
{\small
\[
\left\{
\begin{array}{lll}
\bIf~(c\in HasSubSite(item, l)) & : &
           PF(c)\mul \\ & &
           \STACK{\sumMPD}{\alpha,~c_{l} \in RootsOf(itemCh)} Pp(c_{l},itemCh,m,q), \\
\bIf~(c\in HasChild(item, l)) & : &
             PF(c) \mul \\
            & & \bIf~{\bf (~}\exists c_{l} \in InternOf(itemCh):~Parent?(c,c_{l},l){\bf~)}\\
              & & \bThen~\STACK{\sumMPD}{\alpha} Pp(c_{l},itemCh,m,q)\\
              & & \bElse~~~0. \\
\end{array}
\right.
\]
}
Both cases in this specification must be implemented as explained above 
in order to achieve linearity in $|\An|$ during the second phase of the
algorithm. The time complexity of the algorithm (two phases) is now proportional
to \mbox{$(|\RulesN| + |\An|) \mul n^{3}$}. As mentioned earlier, $\frac{|\RulesN|}{|\An|}$
is very small for DOP~STSGs. Therefore, the time complexity actually approaches
$O(|\An| \mul n^{3})$ as $\frac{|\RulesN|}{|\An|}$ approaches zero. For most DOP STSG
the actual time complexity indeed approaches the linear in STSG size.
This optimization does not result in any change in the space complexity, which remains
$O((|R|+|\An|) \mul n^{2})$.

It is interesting to observe the effect of this optimization in practice.
To this end, I conducted a  preliminary experiment\footnote{
This experiment was conducted with the first implementation
of the MPD algorithm. As most first implementations, it was also suboptimal due to choice of
simple but inefficient data-structures; thus, only the ratios between the CPU-times of
the various versions are of interest here, rather than the absolute CPU-times listed 
in the table. 
It is worth noting that subsequent versions improved the figures for all versions 
substantially (see the experiments in chapter~\ref{CHARSImpExp}).
} comparing various versions of the
algorithm: a linear version in STSG size, a square version and a version
that searches for the child of each address using Binary-Search on ordered
arrays. The results are listed in Table~\ref{Simaantable1}.
The experiments reported in table~\ref{Simaantable1} used the ATIS domain 
Penn Tree-bank version 0.5 (Penn TreeBank Project, LDC) without modifications. 
They were carried out, on a 
{\bf Sun Sparc station 10} with 64 MB RAM, parsing ATIS word-sequences.
The three versions were compared for execution-time by varying STSG sizes
on the same test set of 76 sentences, randomly selected. 
The sizes of the STSGs were varied by varying the allowed maximum depth
of elementary-trees and by projecting only from part of the tree-bank in some
other cases (with a maximum of 750 training trees). 
Average cpu-time  includes parse-forest generation, i.e. both phases.
It is clear that there is a substantial difference in growth of execution-time 
between the three versions as grammar size grows.
%\footnote{A simple minded analysis 
%shows that the square version indeed exhibits execution-times that can be approximated by
%$4\mul (10^{-4}\mul |A|)^{2}$ and the linear indeed $10^{-3}\mul |A|$~!!}. 
Note also that this experiment exemplifies, to some extent, the ratio between $|R|$ and $|A|$ 
for ATIS DOP STSGs. These observations hold also for experiments with DOP on other
domains, reported in chapter~\ref{CHARSImpExp}.
%
%
%
%%%
{\bf
\begin{table}[tb]
\vspace*{1em}
\hrule
\vspace*{0.1em}
\begin{small}
\begin{center}
%\begin{tabular}{|c|c|c|c||c|c|c|}
\begin{tabular}{cccc|ccc}
%\hline
{\footnotesize\bf num.\ of} & $|$\Rules$|$ & $|\An|$ & {\footnotesize\bf Avg.Sen.} & 
%\multicolumn{3}{c|}{Average CPU-secs.} \\
\multicolumn{3}{c}{\footnotesize Average CPU-secs.} \\
{\footnotesize\bf elem.\ trees} &  &  & {\footnotesize Length} & 
{\footnotesize linear} & {\footnotesize Bin.Search} & {\footnotesize Square} \\
\hline
74450 & 870 & 436831 & 9.5 &  445 & 993 & 9143 \\
26612 & 870 & 381018 & 9.5 &  281 & $-$ &  $-$ \\
19094 & 870 & 240619 & 9.5 &  197 & $-$ & 2458 \\
19854 & 870 &  74719 & 9.5 &  131 & 223  & 346 \\
% 1442 & 113 &  5148 & 9.3 &  0.74 & 1.31 & 2.43\\
%\hline
\end{tabular}
\end{center}
\end{small}
\caption{Disambiguation times for various STSG sizes}
\vspace*{0.3em}
\hrule
\label{Simaantable1}
\end{table}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\FSM}{$(Q, \Sigma, S, T, F)$}
%\newcommand{\SFSM}{$(Q, \Sigma, S, T, F, P)$}
\subsection{Extension for disambiguating word-graphs}
\label{SecOptAlg4WGs}
%
The two-phase algorithm for parsing and disambiguating sentences under STSGs
can be easily extended for parsing and disambiguating word-graphs as those
produced by speech recognizers. As mentioned in chapter~\ref{CHDOPinML}
a word-graph is a Stochastic Finite State Machine (FSM). For notation and
definitions on word-graphs, the reader is referred to chapter~\ref{CHDOPinML}.
%%
%\DEFINE{Finite State Machine (FSM):}
%{An FSM is a quintuple \FSM, where $Q$ is a finite set 
%of symbols called the alphabet, $\Sigma$ is a finite set of states,
%$S \in \Sigma$ is the start-state, $F \in \Sigma$ is the target or final state,
%and $T$ is the set of transitions, i.e tuples $<s1,s2,w>$ 
%where $s1, s2 \in \Sigma$ and $w \in Q$.
%}
%%
%\DEFINE{Stochastic FSM (SFSM):}
%{An SFSM \SFSM~ extends an 
% FSM\linebreak
%  \FSM~ 
% with the probability function \mbox{$P:T\lraN (0,1]$}, such that \linebreak
% $\forall l\in\Sigma$:~ \mbox{$\sum_{r\in\Sigma}\sum_{t\in Q} P(<l,r,w>) = 1$}.
%%
%\marginpar{Check this!!}
%%
%}
%%
%\DEFINE{Language of an FSM:}
%{The language of an FSM is the set of all strings 
% from\footnote{$Q^{+}$ denotes the union of all $Q^{n}$, $n\geq 1$. $Q^{*}$ denotes 
%               the set $\{\epsilon\}\cup Q^{+}$.}
% $Q^{+}$ that the FSM {\em accepts}; 
% a string $w_{1}^{n} \in Q^{+}$ is accepted by the FSM \FSM~ iff
% and there are in $T$ transitions 
% \[ <S,s1,w_{1}>, <s_{1},s_{2},w_{2}>, \cdots <s_{n-1},F,w_{n}> \]
% such that for all~ \mbox{$0\leq i \leq n-1$} $S_{i} \in \Sigma$ and $s_{0}$ denotes $S$.
% A sequence of transitions
% $<s_{0},s1,w_{1}>$, $<s_{1},s_{2},w_{2}>$, $\cdots$, $<s_{n-1},s_{n},w_{n}>$,
% where \mbox{$s_{0} = S$} and \mbox{$s_{n} = F$}, is called a {\em derivation}\/ of $w_{1}^{n}$.
% Any sequence of transitions
% $<s_{1},s2,w_{1}>$, $<s_{2},s_{3},w_{2}>$, $\cdots$, $<s_{n},s_{n+1},w_{n}>$ is called a
% {\em path}\/ and
% denoted with the shorter notation $s_{1} s_{2}\cdots s_{n+1}$ \lmdir $w_{1}^{n}$.
%}
%%
%\DEFINE{Language of an SFSM:}
%{The language of \SFSM~ is a set of pairs \mbox{$<{\tt string}, {\tt probability}>$} 
% such that\/ ${\tt string}$ is in the language of \FSM~\linebreak
% and\/ ${\tt probability}$ is the sum of the probabilities
% of all derivations of\/ ${\tt string}$, where the probability of a derivation
% $<s_{0},s1,w_{1}>$, $<s_{1},s_{2},w_{2}>$, $\cdots$, $<s_{n-1},s_{n},w_{n}>$ is defined
% as \mbox{$\prod_{i=1}^{n} P(<s_{i-1},s_{i},w_{i}>)$}. 
% The {\em probability of a path}\/ between two states in the word-graph is defined in the same 
% fashion as the probability of a derivation.
%}
%%
%
\DEFINE{Assumptions:}
{
 In this work we assume FSMs and SFSMs that contain no cycles, 
 i.e. paths $s_{x} \cdots s_{x} $ \lmdir $w_{1}^{n}$, for $n \geq 1$. 
 Due to the preceding assumption we may assume, without loss of generality,
 that the set of states $\Sigma$, of SFSM \SFSM, is equal to the set of numbers 
       \mbox{$\{0,1,\cdots (|\Sigma|-1)\}$}
       such that: 1)~each transition 
       $<s1,s2,w>$ fulfills \mbox{$s1 < s2$}, 2)~the start-state $S$ is~$0$,
       and 3)~the target state is~$(|\Sigma|-1)$.
}
%
Before discussing how to parse and disambiguate word-graphs under DOP STSGs,
it is clarifying to note that a sentence $w_{1}^{n}$ is also a simple word-graph.
The CKY algorithm exploits this by numbering a position between the words $w_{i}$ 
and $w_{i+1}$, for all $1\leq i\leq n$, by the number $i$. It also numbers the
position before the first word by $0$. These are the states of a word-graph with
the transitions $<i-1,i,w_{i}>$, for all \mbox{$1\leq i\leq n$}. Note that in a sentence,
every transition is from a state $i$ to the state $i+1$. In general word-graphs
this is not the case; transitions can be from any state $i$ to any state $j > i$.

Parsing an FSM with a CFG is known in the literature as the problem of computing
the intersection of the two machines; studies of algorithms for conducting this 
intersection are discussed in e.g.~\cite{GJvanNoord}. 
Below I discuss how to extend the two-phase MPD computation algorithm under STSGs for 
word-graphs, i.e. SFSMs. Firstly I discuss how to extend the CKY parser of the first phase 
for this task in a similar fashion to preceding work. After that, I discuss how to
compute the MPD of an SFSM under an STSG, in the second phase of the present 
algorithm.

Assume again that we are given the STSG \stsg = \STSG~ in CNF, and let 
\cfg = \CFG denote the CFG underlying it. Moreover, let $WG$ denote the wordgraph 
\SFSM ~where $\Sigma = $\mbox{$\{0,\cdots M\}$}, $M \geq 1$, 
$Q = \{w_{i} | 1\leq i\leq X\}$, and $S$ denotes~$0$ and $F$ denotes~$M$. 
For the rest of this section, we assume that \mbox{$Q\subseteq $\VT} holds. 
%
\subsubsection{First phase}
Recall that when the CKY algorithm parses the sentence $w_{1}^{n}$ under a
CFG, it maintains the following invariant for every entry $[i,j]$ in its table: 
%
\begin{verse}
  \ITEM{A}{\alpha}{\beta}$\in [i,j]$ if and only if (iff) 
  \mbox{$\RuleM{A}{\alpha\beta}$ \lmdir $w_{i}^{j}\beta$}\/ holds in the CFG at hand.
\end{verse}
%
Both parts of the CKY, {\bf Deduce} and {\bf Init}, maintain this. In particular, the
{\bf Deduce} part also relies in its inference on this invariant when combining a 
partial-derivation
of $w_{i}^{k}$ together with a partial-derivation of $w_{k}^{j}$ into a partial-derivation 
of $w_{i}^{j}$. 

For a word-graph with a set of states \mbox{$\{0,\cdots M\}$}, $M \geq 1$, 
the CKY employs a table as used for a sentence of length $M$. 
The only change in the CKY algorithm is in the {\bf Init} part, which now adds the
items \ITEM{A}{w_{l}}{}, for all $\RuleM{A}{w_{l}} \in \RulesN$, 
to entry \entry{i}{j} if there is a transition $<i,j,w_{l}>$ in the word-graph at hand.
Figure~\ref{FigCKYWGs} shows the CKY algorithm extended for word-graphs.
One can easily see that this extension of {\bf Init} still fulfills the CKY invariant.
A useful property of word-graphs is that if there is a path from state~$i$ to state~$k$
and a path from state~$k$ to state~$j$, then there is a path from state~$i$ to state~$j$.
Therefore, it is easy to prove that the above modest extension of the CKY is sufficient 
to maintain the invariant of the CKY algorithm for parsing word-graphs. The CKY table contains
now a parse-forest consisting of all possible parses of every 
sequence of transitions, i.e. all paths, in the input word-graph. 
% which starts at state~$0$ and finishes at state~$M$.
%
\begin{figure}
\hrule
\begin{tabbing}
{\bf Init:} \=                                           \\
            \> $\forall$ \= ~$<i,j,w>~ \in~ T$    \\
            \>           \> $\forall$ \= ~$\RuleM{A}{w} \in$ \Rules      \\
            \>           \>           \> ~~~add \ITEM{A}{w}{} to $[i,j]$ \\
            \>           \> $\forall$ \= ~$\ITEMN{B}{\beta}{} \in [i, j]$  \\
            \>           \>           \> $\forall~ \RuleM{A}{B C} \in$ \Rules \\
            \>          \>            \> ~~~add \ITEM{A}{B}{C} to $[i, j]$  \\
{\bf Deduce:}\=                  					\\
             \>$\forall$ \= ~$0 \leq i < M$ \AND~ $\forall$~ $i < j \leq M$			\\
             \>          \> ~~~$\forall$\= ~$i < k < j$  \AND~
                                            $\forall~ \ITEMN{A}{B}{C}\in [i, i+k]$ 		\\
             \>          \>             \>~~\bIf~ $\exists$ \ITEM{C}{\alpha}{} $\in [i+k, j]$\\
             \>          \>             \>~~\bThen~ add \ITEM{A}{BC} to $[i, j]$ \\
             \>          \> ~~~$\forall$\= ~$\ITEMN{B}{\beta}{} \in [i, j]$ \AND~
                                            $\forall~ \RuleM{A}{B C} \in$ \Rules \\
             \>          \>             \> ~~add \ITEM{A}{B}{C} to $[i, j]$  \\
\end{tabbing}
\hrule
\caption{CKY algorithm for parsing word-graphs under CFGs in CNF}
\label{FigCKYWGs}
\end{figure}
%

The time-complexity of this extended CKY for word-graphs is a function of the number
of states $M$. Similar to the original CKY, the time-complexity is 
$O(|\RulesN|\mul M^{3})$ and the space-complexity is $O(|\RulesN|\mul M^{2})$. 
Note that the number of transitions between any two states does not affect this
time-complexity. The number of transitions does not play a role in the parsing 
steps taken by the CKY {\bf Deduce} and it only introduces  an additional contant 
of time and space complexity during CKY {\bf Init}. But even this constant is accounted 
for the worst case complexity analysis given above (the $O()$ notation). 
%
%
\subsubsection{Second phase}
%Let $WG$ denote the wordgraph \SFSM where $\Sigma = $\mbox{$\{0,\cdots M\}$}, $M \geq 1$, 
%$Q = \{w_{i} | 1\leq i\leq X\}$, and $S$ denotes~$0$ and $F$ denotes~$M$. 
%
\DEFINE{Intersection derivation:}
{An intersection-derivation (or simply i-derivation) of \stsg~ with $WG$
 is a pair $(D_{stsg},D_{WG})$,
where $D_{stsg}$ is a \stsg~ derivation of the sentence $w_{1}^{n}$, and
$D_{WG}$ is a $WG$ derivation of $w_{1}^{n}$, i.e. 
$D_{WG}$ = \mbox{$0,k_{1},\cdots,k_{m},M$\lmdir $w_{1}^{n}$},
where $\forall 1\leq i\leq m$: $k_{i}\in \Sigma$.
}
\DEFINE{Probability of i-derivation:}
{The probability of the i-derivation $(D_{stsg},D_{WG})$ is equal to the multiplication 
of the probability of $D_{stsg}$ with the probability of $D_{WG}$. 
}
\DEFINE{MPiD:}
{The Most Probable i-Derivation (MPiD) of a word-graph $WG$ under the  STSG 
 \stsg~ is defined as the pair $(D_{stsg},D_{WG})$ with the maximum probability.
}
%
For computing the MPiD of $WG$ under \stsg~ we note that the second phase of the present
algorithm does not discriminate between a word-graph and a sentence; all it sees
is a parse-forest in a CKY table. Therefore, algorithm~\ref{AlgPS} can be
applied for computing the MPiD of an input word-graph without transition probabilities,
i.e. an FSM. For incorporating the probabilities of the transition of an SFSM
word-graph, the algorithm is extended in a very simple manner: for every item
\ITEM{A}{w_{l}}{} in entry \entry{i}{j} the term for $Pp$ is multiplied with
the transition probability $P(<i,j,w_{l}>)$. Figure~\ref{SIMAANAlgWG} exhibits
the specification of this algorithm. A proof of the correctness of this 
algorithm is very simple and will be skipped here.
%
%%%%
\begin{figure}[thb]
\hrule
\[
\begin{array}{rll}
& & \\
P_{mpd}(w_{0}^{n}) \hspf & \hspf = & 
\sumMPD_{\tiny\hspf\TABS
{\ITEM{S}{\alpha}{}$\in \entryN{0}{n}$} 
{$c\in \An(\ITEMN{S}{\alpha}{},~0,~n)$}
{and $Root?(c)$}{}}
Pp(c,~\ITEMN{S}{\alpha}{},~0,~n)\\
\mbox{ } & & \\
%\hspfth
Pp(c,item,i,j) &\hspf =\hspf  &  \hspf \bCase item~\bOf \\
\mbox{ } & & \\
\hspfth
\ITEMN{A}{w_{l}}{} \hspft &\hspfth :\hspfth & \hspfth P(<i,j,w_{l}>)\mul PF(c), \\
\\
\hspfth
\ITEMN{A}{B}{C} \hspft &\hspfth :\hspfth &  \hspfth
  \overbrace{
       \STACK{\sumMPD}{\alpha}
       \STACK{\sumMPD}{c1\in \An(\ITEMN{B}{\alpha}{},i,j)}
        P(c)(c1, 1)\mul
        Pp(c1, \ITEMN{B}{\alpha}{}, i, j)}, \\
\\
\hspfth
\ITEMNM{A}{BC}{} \hspft &\hspfth :\hspfth& \hspfth
\sumMPD_{i < k < j}~Pp(c, \ITEMN{A}{B}{C}, i, k)~\mul
\\
& & 
        \overbrace{
       \sumMPD_{\alpha}
            \sumMPD_{c2\in \An(\ITEMN{C}{\alpha}{}, k, j)}
P(c)(c2, 2)\mul Pp(c2, \ITEMN{C}{\alpha}{}, k, j)}
\end{array}
\]
\caption{Algorithm for computing the MPiD of word-graph $WG$}
\label{SIMAANAlgWG}
\vspace{1em}
\hrule
\end{figure}
%

The algorithm in figure~\ref{SIMAANAlgWG} can be adapted for computing the total
probability of a given word-graph under the given STSG. This can be achieved
by exchanging every $\sumMPD$ with a $\sum$. 

Similar to the original algorithm, the time-complexity when applying the optimization
(which is still valid) is $O(|\An|\mul M^{3})$ and the space-complexity 
is $O(|\An|\mul M^{2})$. The total times-complexity for both phases of the algorithm 
is $O((|R|+|\An|)\mul M^{3})$  and the space-complexity is $O((|R|+|\An|)\mul M^{2})$
%
%
%%%%
% word-graph parsing with CKY
% word-graph probabilities incorporation
% MPD computation with respect to alg~\ref{AlgPS}
% complexity
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{DOPDIS}
%
%
\section{Useful heuristics for a smaller STSG}
\label{SecHeuristics}
%Grammar size gets larger with larger domains and harder applications
%For computing the MPD: note that we can try  to minimize the number of substitutions.
%Or set an upper bound d_
% Explain d_ n_ l_ L_ similar to n-grams

Our practice has shown that as soon as the domains and the applications 
take practical forms, the interesting DOP STSGs acquire non-manageable sizes. In some
cases, these models could not be acquired or executed, even on sizeable machines, 
due to the huge number of elementary-trees (typically exceeding a hundered million
for small domains). And in the few cases where they could be acquired and executed,
various problems were encountered: sparse data effects, extremely slow 
execution-times and extremely small probabilities. A possible solution is to
search for approximations that are manageable.

In analogy to n-gram models, Bod~\cite{RENSDES} suggested to infer DOP STSGs with 
elementary-trees of some maximal depth (i.e. number of edges in longest path). 
In many cases this proved quite useful, e.g. maximum depth four turned out to be
a good approximation in various situations. However, since limiting subtree-depth
to small values (typically depth one or two) simply implies sacrificing accuracy,
one ends up employing ``mid-range" values (e.g.~four or five). For mid-range values
the number of subtrees remains extremely large (depth four already exceeds 
a couple of million for small domains). Therefore, usually limiting subtree-depth 
alone is not effective enough. Next I discuss shortly other similar 
heuristics that are as effective as the upper bound on depth and can be applied
in conjunction with it.

An interesting aspect of the MPD in DOP is a general tendency 
for preferring  shorter derivations involving more probable trees. 
Shorter derivations imply a smaller number of substitutions. 
In general, one can imagine that there is an upper bound 
on the number of substitutions in most probable derivations of 
sentences of a certain domain under some DOP model. 

In practice, this knowledge can be exploited  in two different ways.
Firstly, during training, off line, a smaller size DOP STSG can be projected
from the tree-bank.  This is operationalized through setting an upper bound 
on the number of substitution-sites a DOP STSG's elementary-tree is allowed 
to have; for example, a maximum of two substitution-sites per elementary-tree.
This heuristic has been exploited in many experiments and turned out to reduce
the size of the DOP STSG up to {\em two orders of magnitude}\/ without loss of accuracy
or coverage e.g.~\cite{MyRANLP95,MyRANLPBook,BonnemaEtAl96,DOPNWORep,BonnemaEtAl97}.
And secondly, during the computation of the MPD, an upper 
bound on the number of substitutions can be exploited for pruning derivations
exceeding that upper bound. The latter pruning heuristic has not been applied yet
in our system. In any event, the two heuristics are complementary to each other and
can be applied simultaneously.

Other heuristics in the same spirit turned out to be useful: an upper-bound
on the number of terminals per elementary-tree and an upper bound on the number
of consecutive terminals per elementary-tree. In total, there are currently
four upper bounds in use: on depth (denoted $d$), on the number of 
substitution-sites (denoted $n$), on the number of terminals (denoted $l$) and on the
number of adjacent terminals (denoted $L$). 
These upper bounds are combined together in conjunction during learning a DOP STSG.
In most experiments reported in this thesis these heuristics are employed
in some form or another. 
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%5
%\subsubsection{Advantages}
%0. We still achieve almost |A| time complexity without too
%   much memory-use:
%     Our parser is: |G|n^3 + |A||G|n^{3} = |A|x2x|G|x n^3
%     and this O(|A||G|n^3). Whenever |G| is extremely small
%     compared to |A| and n is large this becomes closer 
%     to O(|A|n^3) !!!
%  So now we can run experiments with huge TSGs very fast !! 
%     A thing that was almost impossible with the direct CKY
%     parser due to memory use in the |A| case. 
%1. No need for extensive use of memory in order to achieve
%   almost |G| time complexity. The rules of the TSG are the
%   subtrees: these are many. In usual CNF transformation
%   the number of different non-terminals in them is 
%   proportional to |NT|x|TSG|, where |NT| is number
%   of non-terminals in underlying CFG and |TSG| is number of
%   subtrees in the TSG. This is because, in order to recognize
%   subtrees we have to be able to recognize that subtrees are
%   units of CNF-CFG rules; this can be achieved only by marking the
%   CFG_CNF rules internal to each subtree with the number of the
%   subtree. This way we face a huge expansion of the memory-use needs.
%   By ECNF approximation this is avoided during the first phase.
%   In the second phase, due to the fact that the first phase 
%   delimits the TSG-parse-space, the application of this knowledge is
%   less bad and does not lead to huge entries.
%2. By parsing with CFG first, we reduce the void derivations
%   in the DOP grammar. Expected to give speed-up and spare memory.
%3. Further, conceptual clarity of a two phases: parsing followed
%    by probabilistic disambiguation. Also clarity of possibilities
%    for combining more linguistically adequate parsers with STSG
%    disambiguators becomes clearer.
%
%\subsubsection{Disadvantages}
% Two phase parsing is expected to be slightly slower for relatively 
%    small TSGs and CFGs. So the parser is specialized in DOP.


==> D-CH_OptAlg4DOP/D-back/OthersAlgs.tex <==
\section{Overview of related work}
\label{SecOthersAlgs}
Historically speaking, parsing Tree-Grammars has been developed mainly within the 
TAG framework. Most work has concentrated on the recognition problem under TAGs 
e.g.~\cite{VijayJoshi85}, \cite{VijayThesis}, \cite{Vijay}. To a much smaller extent, 
some work concentrated on probabilistic disambiguation and probabilistic training 
of some restricted versions of STAGs, e.g.~\cite{SchabesWaters93}. 

The algorithm presented in~\cite{SchabesWaters93} can be used to compute the MPD
of an input sentence under STSGs. Similarly, existing SCFG algorithms based
on CFG parsing algorithms~\cite{ViterbiCFG,Jelinek} can be extended to compute the
MPD for an input sentence under STSGs, as the next section explains. However,
as I argue in that section, none of these algorithms can 
achieve time-complexity linear in STSG size without resulting in huge memory-use.
Moreover, since none of these algorithms is really tailored for the huge DOP STSGs, 
none of them suitably exploits the properties that are typical to these STSGs.\\ 

%Recently, there has been other work dedicated to developing algorithms for the DOP 
%model~\cite{Goodman96,GoodmanDES}. Below we discuss this work briefly.
%
%\subsection{Goodman's DOP SCFG}
Recently, Goodman~\cite{Goodman96,GoodmanDES} presented a new DOP projection mechanism:
rather than projecting a DOP STSG from the tree-bank, Goodman projects from the tree-bank an
equivalent SCFG. The projected SCFG is equivalent to the DOP STSG of that 
tree-bank in the sense that both generate the same parse-space\footnote{
Actually, up to node renaming, there is a homomorphism between the trees of the two grammars.}
and the same parse-probabilities. However, the derivation-spaces of the STSG and the SCFG 
differ essentially. The SCFG implementation of DOP (or DOP SCFG) does not have the notion 
of a subtree and thus
prohibits the computation of such entities that depend on subtrees e.g. the MPD (of the STSG).
However, the SCFG implementation enables fast parsing and computation of the other 
maximization entities of an input sentence. 

Besides the SCFG projection mechanism, \cite{Goodman96,GoodmanDES} presents efficient algorithms 
for computing new maximization entities under the DOP SCFG and studies the plausibility of Bod's
empirical results. The main maximization entity in that work concerns the so-called General 
Labeled Recall Parse (GLRP); the GLRP is the 
parse-tree which maximizes the {\em expectation value of the Labeled Recall rate}\footnote{
A labeled constituent is a  triple $<i,j,A>$, where $w_{i}^{j}$ are the words covered by
the constituent and $A$ is the label of that constituent.
Let be given a parse-tree $T$ selected by a parser for an input sentence and also the correct 
parse-tree $CT$ (i.e. the ultimate goal of the parser) for that sentence.
The Labeled Recall rate is the ratio between the number of correct labeled constituents 
in $T$ and the total number of nodes in $CT$. Roughly speaking, Goodman's algorithm computes
for every labeled constituent in the chart of the input sentence a ``weight";
the weight of a given labeled constituent is the ratio between {\em the product of its 
Inside and Outside probabilities}\/ and the total probability of the input sentence. 
Subsequently, Goodman's algorithm computes the GLRP as that candidate parse (of the input 
sentence) which has the maximum sum of ``weights" of all its labeled constituents.
}. Goodman shows that on the small ATIS, the GLRP achieves exactly the same accuracy as the 
MPP of the DOP STSG (which is equal to the MPP of the DOP SCFG).

A nice property of Goodman's SCFG instantiation of DOP is that it employs the whole
training tree-bank {\em as is}\/ for parsing; this is equal (in the sense mentioned above)
to the DOP STSG as defined in chapter~\ref{CHDOPinML}. This nice quality is also the bottleneck 
of Goodman's implementation\footnote{
Goodman's SCFG has approximately $8\mul N\mul T$ rules, where $T$ is the number of trees
in the tree-bank and $N$ is the average number of words per sentence. For a relatively
small tree-bank of 10000 trees, on average 6 words per sentence, the SCFG has~480000 rules
(about half a million). 
}. Goodman does not offer a way to limit the grammar's subtrees;
this is an essential property for obtaining DOP models under larger tree-banks and 
for avoiding sparse-data effects.  An attempt\footnote{
In personal communication, Goodman has shown that there are such possibilities but that
the number of rules of the SCFG remains very large. Limiting the substitution-sites 
is in fact only a theoretical possibility rather than a practical one.
} at limiting the depth and the number of substitution-sites 
(see section~\ref{SecHeuristics}) of subtrees in Goodman's SCFG, 
immediately results in large SCFGs (hundreds of thousands of different rules). 
As section~\ref{CKYViterbi} explains, such large SCFGs currently form a serious problem 
for parsers.
%Nevertheless, the attractive side of Goodman's implementation of the full DOP 
%model as an SCFG is that it avoids the projection of a possibly exponential number of 
%elementary-trees from a tree-bank. This is 
%is a very promising 
%alternative to Bod's implementation as an STSG~\cite{RENSDES}; essentially, 

Although Goodman's algorithms provide efficient solutions to some problems of
disambiguation under DOP, Goodman's solutions are only suitable for DOP models that 
are represented as SCFGs. In this chapter, I provide efficient solutions to other 
disambiguation problems under STSGs in general, and in particular under DOP STSGs.
%
%consists of the collection of labeled constituents that maximize 
%the {\em expectation value of the Labeled Recall rate of these constituents}\/ 
%``Maximum Constituents Parse" (MCP); 
%the MCP is the parse-tree which maximizes the expected number of 
%correct constituents for a given input sentence\footnote{
%


==> D-CH_OptAlg4DOP/D-back/temp <==
\begin{tabbing}
{\bf Init:} \=                                                          \\
            \> $\forall w_{i}$, $0 < i \leq n$,  	 \\
            \> $\forall$\= \Rule{A}{w_{i}}$\in$\Rules       \\
            \>          \> add \ITEM{A}{w_{i}}{} to $[i-1,i]$ \\
{\bf Deduce:}\=                  					\\
             \> $\forall 0\leq i < n$       			\\
             \> $\forall i\leq j \leq n$			\\
             \> $\forall i < k < j$				\\
             \> $\forall$\= \ITEM{A}{B}{C}$\in [i, i+k]$ 		\\
             \>	         \> if $\exists$\ITEM{C}{\alpha}{}$\in [i+k, j]$\\
             \>          \> then add \ITEM{A}{BC} to $[i, j]$ \\
\end{tabbing


==> D-CH_OptAlg4DOP/Experiments.tex <==
\section{Empirical observations}
\label{SecEmpiric}
The experiments are:
\begin{verbatim}
For tasks: sentence/word-graph parsing and disambiguation
For domains: OVIS, SRI's-ATIS, maybe WSJ
Questions:
      0. quality of parse-space (how often is right parse in the parse-space)
      1. quality of MPD-parse
      2. upper-bound on quality of MPP-parse
      3. quality of probabilistic order of derivation-space (n-MPDs)
         maybe draw a graph: accuracy vs. the number of selected MPD's (n)

   Quality: for each experiment:
            1. exact match 
            2. labeled brackets accuracy and recall
            3. non-labeled brackets
            4. postagging quality
            5. exact sentence-match (for word-graphs)
            6. recall/accuracy words (for word-graphs)
     Also table of means and std

  Other measures:
         1. size of CFG/STSG in DOP STSG
         2. cpu-time CFG/STSG
\end{verbatim}

\subsection{OVIS sentences}
\subsection{OVIS word-graphs}
\subsection{SRI's ATIS sentences}
\subsection{Quality of approximations of the DOP model}
Allow probabilities to remain the same as in the USTSG rather than the limited-depth
DOP model: i.e. even for the limited model use the frequencies normalized with respect
to the whole space rather than the smaller space (this results in probability mass loss). 
Is there any significant change in accuracy ? this is a study of the quality of 
approximating the DOP model using the heuristics as well as the fact that original DOP 
only normalizes in the existence of all subtrees.
%
\subsection{Estimating MPP using MPD-algorithm}
Through retraining the subtrees we obtain new probabilities. How does this model
compare to DOP-MPD ?


==> D-CH_OptAlg4DOP/Heuristics.tex <==
%
\subsection{Successful heuristics}
For various domains and applications (e.g. speech understanding) 










 The sizes of the tree-banks we are facing are getting larger. The training trees are
 getting larger and more complex. So we need some useful ways to constrain the DOP
 models in a way similar to n-grams that are often limited to 3-grams or 2-grams.
 This is done by setting constraints on the form of the subtrees obtained from the
 tree-bank when obtaining a DOP model. Currently, within DOPDIS, we incorporated 
 the following four heuristics:
  1. upper bound on subtree depth (due to Bod) d_
  2. upper bound on number of subs sites in a subtree (Simaan) n_
  3. upper bound on number of words (terminals) in a subtree (Simaan) l_
  4. upper bound on number of adjacent words in a subtree (Simaan) L_
 These heuristics are combined in an AND when obtaining the subtrees.

 Extensive experiments has shown this, especially the depth and the sub sites
 upper bounds to be extremely effective in limiting the number of subtrees
 (list papers and reports showing this effect).

 Interesting points:
 - Why is the upper bound on num of subs-sites the least harmful when computing the MPD ?
    Simply because there is a strong association between the prob of a derivation
    and the number of substitutions that take place in it. So one can assume that
    for a given domain tree-bank there is an upper bound which does not harm the
    space of derivations or probabilities.
 
   One old experiment on ATIS words (without parsing unknown words).
   Showing that results achieved on ATIS are the same even when constraining the
   number of subs-sites. Maybe I should add more experiments ? on OVIS ? on large
   ATIS ?

 - Questions: Compute probability normalization in a constrained DOP grammar w.r.t.
       whole UTSG or w.r.t. constrained STSG DOP. Experiments to check this ?
   Discuss this and maybe show experiments on OVIS and ATIS ?
%%
%
\section{Empirical evaluation}
0.  What is the coverage possible i.e. how often is the right parse found in the
    parse forest anyway ?
1.  Is the probability of the right parse larger or smaller 
    than that of the MPD-predicted parse.
2.  How good are the n-MPDs in predicting the right parse ? 
%
Experiment with this on ATIS, OVIS, ATIS-SRI and maybe even WSJ.
Repeat every experiment 3 to 5 times with independent training/test sets.
%
%
\section{Discussion, open questions and suggestions}
1. Why does MPD work well for Phrase Structure Annotations in the tree-banks which we
  used for our experiments ? Can we provide an explanation for this ?
  Denote the order the parses of a sentence according to their MPDs with the term
  "MPD order of parse-space". Similarly define the ``MPP order of parse-space".
   It seems that under certain circumstances, for many sentences the top of the
   two orders is the same. What circumstances are these and can we derive this fact
   from these circumstances. Note that on the training set sentences the MPD of
   USTSG is equal to the MPP with high probability. 
   Possible observations: MPD is more prone to size of training-set, MPD is more prone
   to errors in training set.

2. When is MPD desirable more than MPP ?
   MPD becomes a better goal than MPP only when the notion of a derivation carries
   with it important clues which a naked parse does not: such as in TAG. Then training
   is done on derivations and parsing has the goal of computing the MPD rather than the
   MPP. The MPD carries a meaning for TAG, while the MPP does not.
3. Suggestion: online constraining of number of substitutions for computing MPD can
   speed up parsing without harming MPD accuracy.


==> D-CH_OptAlg4DOP/OlineOptAlg4DOP.tex <==
\chapter{An optimized algorithm for DOP}
\label{CHOptAlg4DOP}
% mention on what papers this chapter is based
THIS CHAPTER DEALS WITH COMPUTING THE  MPD under STSGs in general using an
optimized deterministic polynomial-time algorithm.
Also computing the probability of a given parse and the probability of
a given sentence. 

Based on the papers~\cite{MyNEMLAP94,MyRANLP95,MyRANLPBook,MyNEMLAPBook,CLASKRep,DOPNWORep}.
This chapter presents the DOPDIS system. The heart of DOPDIS is the 
optimized algorithms for computing the Most Probable Derivation (MPD)
and the Total Probability (TP) of an input sentence (or word-graph).
A short overview of DOPDIS.
DOPDIS is the first system for DOP that computes the MPD/TP
in a deterministic polynomial algorithm, linear is grammar size and up to
100 times faster than Rens's experiments on the same ATIS. DOPDIS is being
used within OVIS. 

%The parser+disambiguator-generator module containing a DOP training-module 
%and transformations of DOP trees into suitable data structures (the RB-STSG
%as presented in the algorithm). The parser module is a CKY parser for
%CFGs. The disambiguation module is based on an STSG probability computation 
%mechanism conducted on the CFG-parse space (maybe we need to mention some
%
\section{An optimized algorithm}
Present it as in the paper.
Improve the complexity analysis.
Exhibit original experiments of speed-up.
%
\section{Extension to word-graphs}
Short description of how to do this.
Provide complexity analysis. And include the number of transitions as
a constant.
%
\section{Extension with word-graph probabilities}
Show how to do this in relation to the optimized algorithm (the exact
place in the algorithm).
%
\section{Heuristic optimizations}
1. the useful d\_n\_l\_L .
2. the useful unknown words construction.
%
\section{Experimental results}
Exhibit the results on ATIS for sentences, on OVIS for sentences.
Show that n_2 in general provides the same results much faster.
For ATIS-SRI sentences and PoSTag sequences. Try WSJ experiments.
%
\section{Discussion and open questions}
1. What about TAG, can we use the same way to achieve faster algorithms ? Discussion.\\
2. Integrating pruning strategies: discuss some possibilities.


==> D-CH_OptAlg4DOP/OlineStructAll <==
  what the chapter presents: 
  Deterministic polynomial-time DOP algorithms
  MPD of a sentence, WG
  probability of a sentence, WG
  probabality of a partial-tree/tree

\section{Introduction}
  Problem description: 
     We are dealing with parsing and disambiguation (not mere recognition)
     Monte-Carlo alg is highly time consuming
     huge probabilistic grammars, so we need algs that are tailored for DOP
  A  possible algorithm, developed independently (Schabes-1993), for TAGs is
     R^2 N3 (can be R^n^3) and does not cash on the special structure 
     of language: relatively 
     small CFG description of the language that can be used to delimit the parse
     space even before very expensive disambiguation.
  In simaan-1994, an alg is described which cashes on this and in simaan-95...
     an algorithm of RN^3 is presented. Linear time in DOP grammar size has proved
     to be an essential part for practice and for experimentation with DOP.
  The system resulting from these algorithms is embedded in the DOPDIS environment.
  Describe DOPDIS and where it is being used.
  CHapter structure.

\section{An optimized polynomial-time algorithm}
  1. Present the MPD algorithm for word-graphs (without probabilities)
     and show how a sentence can be seen as a word-graph.
     a. Without optimization
     b. With optimization
  2. Also computing the prob of a sentence/wg on basis of that algorithm
  3. computing probability of a tree on basis of that algorithm
  4. Allowing speech-recognizer output word-graphs with probabs on the transitions
     (no empty transitions, no cycles). Show how that is done on basis of the algorithm
     above.
 
  One old experiment for showing speed up of linear algorithm.
%
\section{Successful Heuristic optimizations for MPD}
 The sizes of the tree-banks we are facing are getting larger. The training trees are
 getting larger and more complex. So we need some useful ways to constrain the DOP
 models in a way similar to n-grams that are often limited to 3-grams or 2-grams.
 This is done by setting constraints on the form of the subtrees obtained from the
 tree-bank when obtaining a DOP model. Currently, within DOPDIS, we incorporated 
 the following four heuristics:
  1. upper bound on subtree depth (due to Bod) d_
  2. upper bound on number of subs sites in a subtree (Simaan) n_
  3. upper bound on number of words (terminals) in a subtree (Simaan) l_
  4. upper bound on number of adjacent words in a subtree (Simaan) L_
 These heuristics are combined in an AND when obtaining the subtrees.

 Extensive experiments has shown this, especially the depth and the sub sites
 upper bounds to be extremely effective in limiting the number of subtrees
 (list papers and reports showing this effect).

 Interesting points:
 - Why is the upper bound on num of subs-sites the least harmful when computing the MPD ?
    Simply because there is a strong association between the prob of a derivation
    and the number of substitutions that take place in it. So one can assume that
    for a given domain tree-bank there is an upper bound which does not harm the
    space of derivations or probabilities.
 
   One old experiment on ATIS words (without parsing unknown words).
   Showing that results achieved on ATIS are the same even when constraining the
   number of subs-sites. Maybe I should add more experiments ? on OVIS ? on large
   ATIS ?

 - Questions: Compute probability normalization in a constrained DOP grammar w.r.t.
       whole UTSG or w.r.t. contrained STSG DOP. Experiments to check this ?
   Discuss this and maybe show experiments on OVIS and ATIS ?
%%
%
\section{Empirical evaluation}
0.  What is the coverage possible i.e. how often is the right parse found in the
    parse forest anyway ?
1.  Is the probability of the right parse larger or smaller 
    than that of the MPD-predicted parse.
2.  How good are the n-MPDs in predicting the right parse ? 
%
Experiment with this on ATIS, OVIS, ATIS-SRI and maybe even WSJ.
Repeat every experiment 3 to 5 times with independent training/test sets.
%
%
\section{Discussion, open questions and suggestions}
1. Why does MPD work well for Phrase Structure Annotations in the tree-banks which we
  used for our experiments ? Can we provide an explanation for this ?
  Denote the order the parses of a sentence according to their MPDs with the term
  "MPD order of parse-space". Similarly define the ``MPP order of parse-space".
   It seems that under certain circumstances, for many sentences the top of the
   two orders is the same. What circumstances are these and can we derive this fact
   from these circumstances. Note that on the training set sentences the MPD of
   USTSG is equal to the MPP with high probability. 
   Possible observations: MPD is more prone to size of training-set, MPD is more prone
   to errors in training set.

2. When is MPD desirable more than MPP ?
   MPD becomes a better goal than MPP only when the notion of a derivation carries
   with it important clues which a naked parse does not: such as in TAG. Then training
   is done on derivations and parsing has the goal of computing the MPD rather than the
   MPP. The MPD carries a meaning for TAG, while the MPP does not.
3. Suggestion: online constraining of number of substitutions for computing MPD can
   speed up parsing without harming MPD accuracy.

